MINDE: Mutual Information Neural Diffusion Estimation

In this work we present a new method for the estimation of Mutual Information (MI) between random variables. Our approach is based on an original interpretation of the Girsanov theorem, which allows us to use score-based diffusion models to estimate the Kullback Leibler divergence between two densities as a difference between their score functions. As a by-product, our method also enables the estimation of the entropy of random variables. Armed with such building blocks, we present a general recipe to measure MI, which unfolds in two directions: one uses conditional diffusion process, whereas the other uses joint diffusion processes that allow simultaneous modelling of two random variables. Our results, which derive from a thorough experimental protocol over all the variants of our approach, indicate that our method is more accurate than the main alternatives from the literature, especially for challenging distributions. Furthermore, our methods pass MI self-consistency tests, including data processing and additivity under independence, which instead are a pain-point of existing methods.

==> MIperspective.tex <==
While the presentation of this work has started with diffusion models, to derive an \gls{MI} estimator leveraging such models as tools, thanks to our analysis it is also possible to follow back the route, and explain existing diffusion models ... from a \gls{MI} perspective

\textit{Loss numerical instability}. The \textit{classical} diffusion models loss, \Cref{eq:loss} has diverging behaviour. Indeed, as discussed in the literature \cite{kim_bis_2022}, it is necessary to introduce a small truncation time $\tau$ into the loss to avoid numerical problems. We here argue that this behaviour can be straightforwardly interpreted from an information theoretic perspective. In the ideal case where $\tilde{s}_t=s_t$, the quantity in \Cref{eq:loss} corresponds to $\textsc{I}(A,A)$, which, for continuous random variables is equal to $+\infty$. This can be understood by noticing that $\textsc{H}(A\g A)=-\infty$, or by noticing that the measures in the \gls{KL} representation of $\textsc{I}(A,A)$ do not satisfy the absolute continuity requirements. Such numerical issues are alternatively avoided by considering (an estimation of ) the \textit{unconditional} score function, referred to as ideal denoiser in \cite{karras2022}, transforming the loss of \Cref{eq:loss} from $\textsc{I}(A,A)$ onto $\KL{\mu^A}{\tilde{\mu}^A}$.

\textit{Classifier-free guidance}. When considering classifier-free guidance \citep{ho2021classifier} with guidance weight $w$, the expected (over conditioning signals $B$) divergence $\int \KL{\tilde\mu^{A_y}}{\tilde\mu^{A_\emptyset}}\dd\mu^B(y)$ is equal to $w$ times the original mutual information between $A$ and $B$. The weighting of the classifier guidance can be consequently interpreted as an \gls{MI} \textit{enhancer} (at the price of losing faithfulness to the original, unconditional $\mu^A$)

\textit{Implicit info-max representation learning}. Conditional diffusion models often include a parametric preprocessing step of the conditioning signal $E=n(B)$, e.g. a neural network which given a prompt $B$ produces an embedding $E$ \citep{rombach2022}. The methodology presented allow to discuss how such models are approximately doing info-max representation learning. Indeed, the training loss of conditional diffusion models can be expressed as
\begin{equation}\label{eq:infomax}
    \E_{\mu^E}\E_{{\mathbb{P}}^{\mu^{A_E}}}\left[\int\limits_0^T\frac{g^2_{t}}{2}
    \left(\norm{\tilde{s}^{\mu^{[A,E]}}_{t,0}(X_t,E)-\nabla\log \left(\bar{\nu}^{\delta_{X_0}}_{t}(X_t)\right)}^2+c\norm{\tilde{s}^{\mu^A}_{t}(X_t)-\nabla\log \left(\bar{\nu}^{\delta_{X_0}}_{t}(X_t)\right)}^2
    \right)\dd t\right],
\end{equation}
with $A_E$ the conditional random variable $A$ given $E$ and $c>0$. By keeping mapping $n$ from $B$ to $E$ fixed, and optimizing w.r.t. , it is possible to show that \Cref{eq:infomax} can be rewritten in the form of $\textsc{I}(A;n(B;\psi)+\text{const}(\psi)$. Then, optimizing w.r.t. to $\psi$ effectively maximizes the information flow between $A$ and learnt mapping for the conditioning signal. In practice, neither the optimization of $\theta$ is perfect, nor the update of parameters $\psi$ is asynchronous. However, we still claim that the considered \gls{MI} perspective would allow ...



\subsection{Image text \gls{MI}}
Generative diffusion models can be interpreted as \textit{recursive} schemes in which starting from pure noise, at each iteration refinements are applied until a sample from the data distribution is obtained. 
It has recently been observed in the text conditional image generation (image $A$, text prompt $B$), that the role of the text prompt throughout the iterative scheme has not constant importance. Indeed: \textit{
At the early sampling stage, when the input data to the denoising network is closer to the random noise, the diffusion
model mainly relies on the text prompt to guide the sampling
process. As the generation continues, the model gradually
shifts towards visual features to denoise images, mostly ignoring the input text prompt} \citep{balaji2022ediffi}. Such claim has been motivated by carefully engineered metric analysis (self and cross attention maps between images and text, as a function of the generation time) and visual inspection of the change in generated images when switching the prompt at different stages of the refinement. 

Using the proposed methodology, it is possible to perform the same analysis leveraging clearly interpretable information theoretic quantities. In particular, we analyze the conditional mutual information $\textsc{I}(A,B\g X_t)$, being $X_t$ the result of the generation process at time $t$ (remember the time runs backward from $T$ to $0$, and consequently $A=X_0$). Such metric quantifies, given observation of the result of generation process up to time $t$, how much information the prompt $B$ still carries about the final generated image $A$. Clearly, when $t=T$, the initial sample is independent on both $A$ and $B$. Consequently, the conditional mutual information will coincide with $\textsc{I}(A,B)$. On the other extreme, a small $t$ implies that all the relevant semantic information has been already generated, and the prompt $B$ won't play any role in any further refinement.

We present results on the xx dataset, with the yy pretrained model in Figure figfig. Interestingly, the plot shows exactly the expected behaviour, corroborating the idea that mutual information can be adopted as an exploratory tool for complex high dimensional data.


==> benchmark.tex <==
\section{Benchmark Description}
\label{apdx:bench}
In this Section, we provide additional details of the benchmark considered in the experimental section \Cref{sec:experiments}. Following \cite{czyz2023beyond}, we use the same settings to generate the 40 tasks. Samples are generated from a \textbf{base distribution} and are post-processed through some non-linear \textbf{transformations}. Hereafter, we report {\textbf{verbatim}} the descriptions of the tasks of the benchmark reported in appendix D3 of \cite{czyz2023beyond}, to aid the reader by making the document self-consistent.





\subsection{Task Descriptions \citep{czyz2023beyond}}\label{appendix:subsection:task-descriptions}

\paragraph{Bimodal Variables} Consider a r.v.\ $X$ distributed according to a Gaussian mixture model with CDF $F = w_1F_1 + w_2F_2$, where $F_1$ and $F_2$ are CDFs of two Gaussian distributions and $w_1$ and $w_2$ are positive weights constrained as $w_1 + w_2 = 1$.
The CDF is everywhere positive, continuous, and strictly increasing.
Hence, it has an inverse, the quantile function, $F^{-1}\colon (0, 1)\to \mathbb R$, which is continuous and injective as well. %(see~Lemma \ref{lemma:increasing-continuous-bijections-are-homeo}).

Thus, we can define r.v. $X' = F^{-1}(X)$, where $ X \sim \mathcal{U}(0, 1)$ and $I(X;Y) = I(X';Y)$ for every r.v. $Y$.
We generated two CDFs of Gaussian mixtures and implemented a numerical inversion in JAX \citep{jax2018github} defining both $X'$ and $Y'$ to follow a bimodal distribution.

For the experimental values, we used
\begin{align*}
    F_X(x) &= 0.3 F(x) + 0.7 F(x-5)\\
    F_Y(y) &= 0.5 F(x+1) + 0.5 F(x-3),
\end{align*}
where $F$ is the CDF of the standard normal distribution $\mathcal N(0, 1)$.


\paragraph{Wiggly Mapping} As the ``wiggly mapping'' we used
\begin{align*}
    w_X(x) &= x + 0.4 \sin x + 0.2\sin(1.7x + 1) + 0.03 \sin(3.3x - 2.5)\\
    w_Y(y) &= y - 0.4\sin(0.4y) + 0.17\sin(1.3y + 3.5) + 0.02\sin(4.3 y - 2.5) 
\end{align*}
%and we used visualisations to make sure that they do not heavily distort the distribution.

\paragraph{Additive Noise}
For the additive noise model of $Y=X+N$ where $X\sim \mathrm{Uniform}(0, 1)$ and $N\sim \mathrm{Uniform}(-\epsilon, \epsilon)$ it holds that
\[
I(X;Y) = 
\begin{cases}
    \epsilon - \log (2\epsilon) & \text{if } \epsilon \le 1/2\\
    (4\epsilon)^{-1} & \text{otherwise}
\end{cases}
\]
implying that $I(X;Y)=1.7$ for $\epsilon=0.1$ and $I(X;Y)=0.3$ for $\epsilon=0.75$.

\paragraph{Swiss Roll Embedding}
Consider a bivariate distribution $P_{XY}$ with uniform margins $X\sim \text{Uniform}(0, 1)$ and $Y\sim \text{Uniform}(0, 1)$ and $I(X;Y)=0.8$.
The Swiss roll mapping is an embedding $i\colon (0, 1)^2\to \mathbb R^3$ given by $i(x, y) = (e(x), y)$, where $e\colon (0, 1) \to \mathbb R^{2}$ is given by
\begin{equation*}
     e(x) = \frac{1}{21}(t(x) \cos t(x),
     t(x)\sin t(x), \qquad
     t(x) = \frac{3\pi}{2}(1+2x).
\end{equation*}
Note that $P_{X'Y'}$ does not have a PDF with respect to the Lebesgue measure on $\mathbb R^3$.
%We visualise the Swiss roll distribution in Fig.~\ref{fig:distribution-visualisation}.

\paragraph{Spiral Diffeomorphism}
%For the precise definition and properties of the general spiral diffeomorphism consult Appendix~\ref{appendix:spirals}.

In our benchmark we applied the spiral $x\mapsto \exp(v A ||x||^2)x$ to both $X$ and $Y$ variables.
We used an $m\times m$ skew-symmetric matrix $A_X$ with $(A_X)_{12} = -(A_X)_{21} = 1$ and an $n\times n$ skew-symmetric matrix $A_Y$ with $(A_Y)_{23} = -(A_Y)_{32} = 1$.
Each of these effectively ``mixes'' only two dimensions.

The speed parameters $v_X$ and $v_Y$ were chosen as $v_X = 1/m$ and $v_Y = 1/n$ to partially compensate for the fact that if $X\sim \mathcal N(0, I_m)$, then $||X||^2\sim \chi^2_m$ and has mean $m$.

\paragraph{Multivariate Student} Let $\Omega$ be an $(m+n)\times (m+n)$ positive definite dispersion matrix and $\nu$ be a positive integer (the degrees of freedom).
By sampling an $(m+n)$-dimensional random vector $(\tilde X, \tilde Y)\sim \mathcal N(0, \Omega)$ and a random scalar $U\sim \chi^2_{\nu}$ one can define rescaled variables $X=\tilde X \sqrt{\nu/U}$ and $Y=\tilde Y\sqrt{\nu/U}$, which are distributed according to the multivariate Student distribution.
For $\nu=1$ this reduces to the multivariate Cauchy distribution (and the first two moments are not defined), for $\nu=2$ the mean exists, but covariance does not, and for $\nu > 2$ both the mean and covariance exist, with
\(
    \mathrm{Cov}(X, Y)= \frac{\nu}{\nu-2}\Omega,
\)
so that the tail behaviour can be controlled by changing $\nu$. In particular, for $\nu \gg 1$ because of the concentration of measure phenomenon $U$ has most of its probability mass around $\nu$ and the variables $(X, Y)$ can be well approximated by $(\tilde X, \tilde Y)$.

\citep{arellano2013shannon} proved that $I(X;Y)$ can be computed via the sum of the mutual information of the Gaussian distributed basis variables and a correction term, i.e., 
\(
    I(X;Y) = I(\tilde X;\tilde Y) + c(\nu, m, n),
\)
where
\begin{align*}
    c(\nu, m, n) &= f\left(\nu\right) {+} f\left(\nu {+} m {+} n\right) {-} f\left(\nu {+} m\right) {-} f\left(\nu {+} n\right),& 
    f(x) &=  \log \Gamma\left(\frac{x}{2}\right) - \frac{x}{2}\psi\left(\frac{x}{2}\right),
\end{align*}
and $\psi$ is the digamma function.

Contrary to the Gaussian case, even for $\Omega=I_{m+n}$, the mutual information $I(X;Y)=c(\nu, m, n)$ is non-zero, as $U$ provides some information about the magnitude.
In the benchmark we use this dispersion matrix to quantify how well the estimators can use the information contained in the tails, rather than focusing on estimating the Gaussian term.

\subsection{Covariance Matrix Family}
\label{section:covariance-matrix}
We generated jointly multivariate normal variables $X=(X_1, \dotsc, X_m)$ and $Y=(Y_1, \dotsc, Y_n)$ with the following procedure.

Consider i.i.d. Gaussian variables

\[U_\mathrm{all}, U_X, U_Y, Z_1, \dotsc, Z_K, E_1\dotsc, E_m, F_1, \dotsc, F_n, E'_{m-K}, \dotsc, E'_m, F'_{n-K}, \dotsc, F'_n \sim \mathcal{N}(0, 1).\]

Now let $\epsilon_X, \epsilon_Y, \eta_X, \eta_Y, \alpha, \beta_X, \beta_Y, \lambda \in \mathbb R$ be hyperparameters and for $l = 1, 2, \dotsc, K$ define
\[X_l = \epsilon_X E_l + \alpha U_\mathrm{all} + \beta_X U_X + \lambda Z_l,\quad Y_l =  \epsilon_Y F_l + \alpha U_\mathrm{all} + \beta_Y U_Y + \lambda Z_l,\]
for $l = K+1, \dotsc, m$ define
\[X_l = \epsilon_X E_l + \alpha U_\mathrm{all} + \beta_X U_X + \eta_X E'_l\]
and for $l = K+1, \dotsc, n$ define
\[
Y_l = \epsilon_Y F_l + \alpha U_\mathrm{all} + \beta_Y U_Y + \eta_Y F'_l.
\]

The interpretation of the hyperparameters is the following:
\begin{enumerate}
    \item $\alpha$ contributes to the correlations between all the possible pairs of variables.
    \item $\beta_X$ contributes to the correlations between the $X$ variables.
    \item $\beta_Y$ contributes to the correlations between the $Y$ variables.
    \item $\lambda$ gives additional ``interaction strength" between pairs of variables $X_l$ and $Y_l$ for $l = 1, \dotsc, K$.
    \item $\epsilon_X$ and $\epsilon_Y$ control part of the variance non-shared with any other variable.
    \item $\eta_X$ and $\eta_Y$ can be used to increase the variance of $X_l$ and $Y_l$ for $l > K$ to match the variance of variables $l\le K$ due to the $\lambda$.
\end{enumerate}
  
Every term of the covariance matrix is easy to calculate analytically:
\[
Cov(X_i, X_j) 
= \alpha^2 + \beta_X^2 + \mathbf{1}[i=j] \big(\epsilon_X^2 +  \lambda^2 \mathbf{1}[i \le K] + \eta_X^2 \mathbf{1}[i>K] \big)
\]

\[
Cov(Y_i, Y_j) = \alpha^2 + \beta_Y^2 + \mathbf{1}[i=j] \big(\epsilon_Y^2 + \lambda^2 \mathbf{1}[i \le K] + \eta_Y^2 \mathbf{1}[i>K] \big)
\]

$Cov(X_i, Y_j) = \alpha^2 + \lambda^2 \mathbf{1}[i=j] \mathbf{1}[i\le K]$


In the following, we analyse some special cases.

\paragraph{Dense Interactions}

Consider $\lambda = \eta_X = \eta_Y = \beta_X = \beta_Y = 0$ and write $\epsilon := \epsilon_X = \epsilon_Y$. We have
$\mathrm{Cov}(X_i, X_j) = \mathrm{Cov}(Y_i, Y_j) = \alpha^2 + \epsilon^2 \mathbf{1}[i=j]$
$\mathrm{Cov}(Y_i, Y_j) = \alpha^2$

Hence, between every pair of distinct variables we have the same correlation $\frac{\alpha^2}{\alpha^2 + \epsilon^2}$.

\paragraph{Sparse Interactions}

Consider $\alpha=0$, $\epsilon := \epsilon_X = \epsilon_Y$, $\eta_X = \eta_Y = \lambda$ and $\beta_X = \beta_Y = 0$

$Cov(X_i, X_j) = \mathrm{Cov}(Y_i, Y_j) = \mathbf{1}[i=j] (\epsilon^2 + \lambda^2) $

$Cov(X_i, Y_j) = \lambda^2 \mathbf{1}[i=j] \mathbf{1}[i\le K]$

All the variables have the same variance, but the covariance structure is now different. Between (distinct) $X_i$ and $X_j$ the correlation is zero and similarly for (distinct) $Y_i$ and $Y_j$.

Correlations between $X_i$ and $Y_j$ are zero unless $i=j\le K$, when $Cor(X_i, Y_i)=\lambda^2 / (\epsilon^2 + \lambda^2)$.





% \textbf{Bimodal Variables}

% Consider a random variable $X$ distributed according to a Gaussian mixture model with
% CDF $F = w_1 F_1 + w2F2$ , where F1 and F2 are CDFs of two Gaussian distributions and w1 and
% w2 are positive weights constrained as w1 + w2 = 1. The CDF is everywhere positive, continuous,
% and strictly increasing. Hence, it has an inverse, the quantile function, F
% −1
% : (0, 1) → R, which is
% continuous and injective as well (see Lemma D.1). Thus, we can define r.v. X′ = F
% −1
% (X), where
% X ∼ Uniform(0, 1) and I(X; Y ) = I(X′
% ; Y ) for every r.v. Y . 

% %We generated two CDFs of Gaussian mixtures and implemented a numerical inversion in JAX [Bradbury et al., 2018] defining both X′ and Y to follow a bimodal distribution.

% \paragraph{Multivariate Normal:} characterized by correlation structure which corresponds to a “dense” interaction or a sparse interation "2-pair". 




% \textbf{Multivariate Student}, which can be to evaluate the capacity of the estimators in capturing \gls{MI} for heavy tailed distributions.
% \end{itemize}
% \paragraph{Transformations:}
% \begin{itemize}
%     \item 
% \textbf{Bimodal Variable}. Corresponds to the application of the inverse CDF of a two-component Gaussian mixture model to correlated variable.
%     \item \textbf{Uniform Margins} apply the Gaussian  CDF to a Gaussian distribution.
%     \item \textbf{Half-Cube Map} homeomorphism $h(x)=|x| \frac{3}{2} \text{sign} x$ is a transformation which lenghthen the distribution length.
%     \item \textbf{Asinh Mapping } An inverse hyperbolic sine function  $asin (x) = \log (x + \sqrt{1+x^2} )$  which shorten the distribution tail length.
%     \item \textbf{Wiggly Mapping}  a transformation which models non-uniform lenghtscales
%     $w(x) = x + \sum a_i \sin ( w_i x + \phi_i)  \quad , \sum |a_i w_i| <1$Variable
%     \item \textbf{Additive Noise} The mutual information of the sum of a sample $X \sim Uniform(0,1)$   with a uniform noise $N \sim Uniform(-\epsilon,\epsilon)$  accepts an analytical solution 
%     \item \textbf{Swiss Roll Embedding} One dimensional uniform sample can be embedded using the Swiss roll embedding into a two dimensional sample.
% \end{itemize}


% The multivariate normal and multivariate Student distributions can be transformed using the mappings described above
% to each axis separately. We use the package \textit{benchmark-mi}\footnote{\url{https://github.com/cbg-ethz/bmi}} to sample from the different distribution tasks.




\paragraph{Preprocessing}
Across all the experiments, we apply an element wise standardization using the mean and standard deviation calculated from the tasks samples.


==> divergences.tex <==
In this Section we proceed to explain how to use \Cref{kl_formula_sm} for various divergences estimation other than the KL divergence between two measures $\nu^{A,B}_0$. This includes, but is not limited to, entropy of a random variable and mutual information estimation.


\subsection{Entropy estimation}
In many applications, estimation of the entropy associated to a given density $\nu^A_0$, $\textsc{H}(\nu^A_0)$ is important. In the considered framework, it is sufficient to know the score function $s^A_t(x)$ to estimate it. Indeed, the following simple equality holds

\begin{equation}
    \KL{\nu^A_0}{\nu^B_0=\mathcal{N}(0,\sigma^2)}=-\textsc{H}(\nu^A_0)-\int \dd \nu^A_0(x)\log \mathcal{N}(x;0,\sigma^2)=-\textsc{H}(\nu^A_0)+\frac{1}{2}\log(2\pi \sigma^2)-\frac{\E_{\nu^A_0}\left[X_0^2\right]}{2\sigma^2},
\end{equation}
where $\mathcal{N}(x;m,\sigma^2)$ stands for the standard Gaussian distribution with mean $m$ and variance $\sigma$. Consequently, rearranging, we notice that estimation of the entropy is possible through 
\begin{equation}
\textsc{H}(\nu^A_0)=-e_T(\nu^A_0,\mathcal{N}(0,\sigma^2))+\frac{1}{2}\log(2\pi \sigma^2)-\frac{\E_{\nu^A_0}\left[X_0^2\right]}{2\sigma^2}.
\end{equation}

First, the score function associated to the forward process starting from $\mathcal{N}(0,\sigma^2)$ is known:
\begin{equation}
s^B_t(x)= -\frac{x}{\chi(t)},\quad \chi(t)=\exp\left(2\int_0^tf(s)\dd s\right)\sigma^2+\exp\left(2\int_0^tf(s)\dd s\right)\int_0^t \exp\left(-2\int_0^sf(r)\dd r\right) g^2(s)\dd s.
\end{equation}
%Notice that in many popular \gls{SDE} parametrizations \cite{song2020}, $g^2(t)=-f(t)$, and consequently we simply have $\chi(t)$
Second, whenever $T$ is large enough $\nu^A_T\simeq \mathcal{N}(0,1)$, independently on the chosen value of $\sigma$. Consequently $\KL{\nu^A_T}{\nu^B_T}\simeq \KL{\mathcal{N}(0,1)}{\mathcal{N}(0,\chi(T))}$, being the divergence between two Gaussian distributions, has analytically known value.
Given knowledge of $s^A_t(x)$, computation of $e_T(\nu^A_0,\mathcal{N}(0,\sigma^2))$ is straightforward.

Depending on the selection of the value of $\sigma^2$ further simplifications are possible to drop the unknown (but easily estimable) value $\E_{\nu^A_0}\left[X_0^2\right]$. Indeed, when $\sigma^2\gg \E_{\nu^A_0}\left[X_0^2\right]$,
\begin{equation}\label{entropy_est}
\textsc{H}(\nu^A_0)\simeq -e_T(\nu^A_0,\mathcal{N}(0,\sigma^2))+\frac{1}{2}\log(2\pi \sigma^2).
\end{equation}

{\color{red} Different combination of $T,\sigma$ will probably impact differently the variance of the estimation}

\subsection{Likelihood estimation}

Given a pretrained diffusion model \cite{song2020}, there are two possibilites to compute the log-likelihood of a given datapoint. First, use the \gls{ODE} version of the diffusion process and integrate numerically the \gls{ODE} and the gradients of the drift terms (extremely expensive).
Second, leverage the result in \cite{huang2021variational} (eq. 25), where no backward diffusion simulation is necessary, but trace Hessians of score are still necessary. 
Third, novel until now, use our methodology. Notice that our result can be interpreted as an extension of the results in \cite{kong2023information}.

The idea is the following: provided $\sigma$ is small enough (but not zero)
\begin{equation}
    \log \nu^B_0(y)\simeq \E_{\mathcal{N}(y;\sigma^2)}\left[\log \nu^B_0(x)\right]=-\KL{\nu^A_0=\mathcal{N}(y;\sigma^2)}{\nu^B_0}+\textsc{H}(\nu^A_0)
\end{equation}

Also in this case, since $\nu^A_0$ is Gaussian, both its associated score function and its entropy are analytically known. Then

\begin{equation}
    \log \nu^B_0(y)\simeq e_T(\mathcal{N}(y;\sigma^2), \nu^B_0)+\textsc{H}(\nu^A_0)
\end{equation}

==> multitime_diff.tex <==
%\subsection{Masked diffusion models}\label{sec:multitime}





==> multitime_diff_backup_newer.tex <==
\subsection{Multi-time diffusion models}

In this work, we are interested in estimating the \gls{MI} between different variables. This implies, as clarified later in \Cref{sec:mutualinfo}, the need to estimate quantities associated to the joint ($\mu^{[A,B]}$), conditional ($\mu^{A\g B=y}$, where in product representation $\mu^{[A,B]}=\int \mu^{A\g B=y}\dd\mu^{B}(y)$) and marginal measures (the already introduced $\mu^{A},\mu^{B}$). Consequently, we will need to estimate the associated score functions. Instead of considering separate diffusion processes we consider a recently introduced \textbf{family} of diffusion processes \citep{bounoua2023multimodal}, which encompasses as particular cases the ones of interest. Consider the following \gls{SDE} 
\begin{equation}\label{eq:diffsdesjoint}
    \begin{cases}
    \dd \left[X_t,Y_t\right]^\top =f_t[\alpha X_t,\beta Y_t]^\top \dd t+ g_t\left[\alpha \dd W_t,\beta \dd W'_t\right]^\top,\\
    [X_0,Y_0]^\top\sim \mu^{[A,B]},
    \end{cases}
\end{equation}
with extra parameters $\alpha,\beta\geq 0$.
This \gls{SDE} is a natural extension of \Cref{eq:diffsdes}, when considering joint evolution of the variables $X_t,Y_t$, starting from the joint measure $\mu^{[A,B]}$, with overall path measure $\mathbb{P}^{[A,B]}$. The two extra coefficients $\alpha,\beta\geq 0$ effectively modulate the \textit{speed} at which the two portions $X_t,Y_t$ of the process diffuse towards their steady state. In this work, out of all the possible values for $\alpha,\beta$, we are interested in some particular cases. More precisely, we either consider $\alpha=\beta=1$, which corresponds to a \textit{classical} simultaneous diffusion, or the configurations $\alpha=1,\beta=0 / \alpha=0,\beta=1 $. %(and the corresponding combination when fixing $\beta=1$).
The last two configurations correspond to diffusions in which either the variable $Y_t$ or $X_t$ remain constant throughout all the diffusion. As clarified hereafter, this will be used for conditional measures.

\begin{comment}
\begin{equation}\label{eq:diffsdesjoint_2}
    \begin{cases}
    \dd \left[X_t,Y_t\right]^\top =f_t[X_t,{\color{red} 0\times}Y_t]^\top \dd t+ g_t\left[\dd W_t,{\color{red} 0\times}\dd W'_t\right]^\top,\\
    [X_0,Y_0]^\top\sim \mu^{[A,B]},
    \end{cases}
    \begin{cases}
    \dd \left[X_t,Y_t\right]^\top =f_t[X_t,{\color{red} \infty\times}Y_t]^\top \dd t+ g_t\left[\dd W_t,{\color{red} \infty\times}\dd W'_t\right]^\top,\\
    [X_0,Y_0]^\top\sim \mu^{[A,B]}.
    \end{cases}
\end{equation}



, which evolves according to the following \gls{SDE} 
\begin{footnotesize}
\begin{equation}\label{eq:diffsdesjoint}
    \begin{cases}
    \dd \left[X_t,Y_t\right]^\top =f_t[X_t,Y_t]^\top \dd t+ g_t\left[\dd W_t,\dd W'_t\right]^\top,\\
    [X_0,Y_0]^\top\sim \mu^{[A,B]}.
    \end{cases}
\end{equation}
\end{footnotesize}
The score function $s^{[A,B]}_t(x,y)$ materializes in the reverse process of \Cref{eq:diffsdesjoint}, the \gls{SDE} corresponding to the reversed path measure $\hat{\mathbb{P}}^{[A,B]}$.
\end{comment}


Reminiscent of the effective modulation of evolution speed of the two variables, given by the parameters $\alpha,\beta$, we now introduce the concept of \textit{multi-time} score functions $s^{[A,B]}_{t; (\alpha,\beta)}(x,y)$, the score functions associated to \Cref{eq:diffsdesjoint}. This new notation allows to efficiently describe joint and conditional scores, as we show next.
First, we notice that when $\alpha=\beta=1$, the double argument indicates that both variables diffuse at the same rate. In this case, the joint score $s^{[A,B]}_{t;(1,1)}(x,y)$ simply correspond to the score of a diffusion process on both variables $A,B$. %, i.e.,
Consider instead a diffusion process on the variable $A$, where initial conditions are drawn conditionally on the event $B=y$, that is from the measure $\mu^{A\g B=y}$ (in product representation $\mu^{[A,B]}=\int \mu^{A\g B=y}\dd\mu^{B}(y)$). The score associated to such a conditional diffusion, %$\nabla_x\log \left(\bar\nu^{A\g B=y}_t(x)\mu^{B}(y)\right)$ 
corresponds to the $x-$part of multi-time score $s^{[A,B]}_{t;(1,0)}(x,y)$. {\color{red} In summary a the family of multitime score functions contains the information for the joint and conditional cases. This will allow lighter presentation of the methodology and provide to be useful in the actual training of the proposed method.}


==> mutual_info_backup.tex <==
In this Section we propose our new \gls{MI} estimator, which we name \gls{MINDE}. It is important to clarify that the proposed methodology encompasses a \textit{family} of techniques, where different choices are dictated by the possible availability of pretrained models and/or computational constraints. 


As starting point for our discussion, we recognize that the \gls{MI} between two random variables $A,B$ has several equivalent expressions, among which \Cref{eq:mi_0,eq:mi_1,eq:mi_2,eq:mi_3,eq:mi_4}. On the left hand side of these set of columns we report classically known equal formulations for the \gls{MI}, while on the right hand side we write the computation using the estimators (the equality should be assumed to be valid up to the estimation errors described in the previous Sections). Notice that complete details are provided throughout this Section.
\begin{comment}
\begin{minipage}{.48\textwidth} %
\begin{alignLetter}
    &\textsc{I}(A,B)=\KL{\mu^{[A,B]}}{\mu^{A}\mu^{B}}= \label{eq:mi_0}\\
    &\int \KL{\mu^{A\g B=y}}{\mu^{A}} \dd\mu^{B}(y)= \label{eq:mi_1}\\
    &\textsc{H}(A)-\textsc{H}(A\g B)=\textsc{H}(B)-\textsc{H}(B\g A)= \label{eq:mi_2}\\
    &\textsc{H}(A,B)-\textsc{H}(A\g B)-\textsc{H}(B\g A)= \label{eq:mi_3}\\
    &\textsc{H}(A)+\textsc{H}(B)-\textsc{H}(A,B) \label{eq:mi_4}
\end{alignLetter}
\end{minipage}
\begin{minipage}{.48\textwidth} %
%\begin{table}[ht]
%\small
%\centering
\hspace*{0.1cm}
\begin{tabular}{|c|c|c|}
\hline
  & \textbf{Conditional} & \textbf{Joint} \\ \hline
Pre-trained & Available & Scarce\\ \hline
$I(A,B)$ & Yes & Yes\\ \hline
$H(A)$ & Yes & Yes\\ \hline
$H(A\mid B)$ & Yes & Yes\\ \hline
$H(B)$ & No & Yes\\ \hline
$H(A,B)$ & No & Yes\\ \hline
Scalability (\# rvs) & Hard & Simple\\ \hline
\end{tabular}
\captionof{table}{Summary of our methods.}\label{tableMI}
%\end{table}
\end{minipage}%

\end{comment}

\begin{footnotesize}
\begin{alignLetter}
    \KL{\mu^{[A,B]}}{\mu^{A}\mu^{B}}=&e(\mu^{[A,B]},\mu^{A}\mu^{B})= \label{eq:mi_0}\\
    \int \KL{\mu^{A\g B=y}}{\mu^{A}} \dd\mu^{B}(y)=& \int e(\mu^{A\g B=y},\mu^{A})\dd\mu^{B}(y) =\label{eq:mi_1}\\
    \textsc{H}(A)-\textsc{H}(A\g B)=& -e(\mu^{A},\GaussM{\sigma})+\int e(\mu^{A\g B=y},\GaussM{\sigma})\dd\mu^{B}(y)\label{eq:mi_2}\\
    \textsc{H}(A,B)-\textsc{H}(A\g B)-\textsc{H}(B\g A)=& -e(\mu^{[A,B]},\GaussM{\sigma})+\int e(\mu^{A\g B=y},\GaussM{\sigma})\dd\mu^{B}(y)+\int e(\mu^{B\g A=x},\GaussM{\sigma})\dd\mu^{A}(x)=\label{eq:mi_3}\\
    =&\E_{\mathbb{P}^{[A,B]}}\left[\int\limits_0^T\frac{g^2_{t}}{2} \left[\norm{{s}^{[A,B]}_{t;(1,1)}([X_t,Y_t])-[s^{[A,B]}_{t;(1,0)}(X_t,Y_0),s^{[A,B]}_{t;(0,1)}(X_0,Y_t)] }^2\right]\dd t\right] \label{eq:mi_3inner}\\
    \textsc{H}(A)+\textsc{H}(B)-\textsc{H}(A,B)=&-e(\mu^{A},\GaussM{\sigma})-e(\mu^{B},\GaussM{\sigma}) +e(\mu^{[A,B]},\GaussM{\sigma})\label{eq:mi_4}
\end{alignLetter}
\end{footnotesize}


\begin{comment}
\begin{alignLetter}
    \KL{\mu^{[A,B]}}{\mu^{A}\mu^{B}}=&e(\mu^{[A,B]},\mu^{A}\mu^{B})= \label{eq:mi_0}\\
    \E_{\mu^{B}}\left[\KL{\mu^{A\g B=y}}{\mu^{A}}\right]=& \E_{\mu^{B}}\left[e(\mu^{A\g B=y},\mu^{A})\right]=\label{eq:mi_1}\\
    \textsc{H}(A)-\textsc{H}(A\g B)=& -e(\mu^{A},\GaussM{\sigma})+\E_{\mu^{B}}\left[e(\mu^{A\g B=y},\GaussM{\sigma})\right]\label{eq:mi_2}\\
    \textsc{H}(A,B)-\textsc{H}(A\g B)-\textsc{H}(B\g A)=& -e(\mu^{[A,B]},\GaussM{\sigma})+\E_{\mu^{B}}\left[e(\mu^{A\g B=y},\GaussM{\sigma})\right]+\int e(\mu^{B\g A=x},\GaussM{\sigma})\dd\mu^{A}(x)\label{eq:mi_3}\\
    \textsc{H}(A)+\textsc{H}(B)-\textsc{H}(A,B)=&-e(\mu^{A},\GaussM{\sigma})-e(\mu^{B},\GaussM{\sigma}) +e(\mu^{[A,B]},\GaussM{\sigma})\label{eq:mi_4}
\end{alignLetter}
\end{comment}
%Then, we present several alternatives to leverage the methodology introduced in \Cref{sec:diffusion}, and apply it to compute the \gls{MI} according to its various formulations. 
Our methods either capitalize on pre-trained diffusion models, or require training from scratch, and come with a variety of properties. %, as summarized in \Cref{tableMI}.
\begin{comment}
\begin{table}[ht]
\small
\centering
\begin{tabular}{|c|c|c|}
\hline
  & \textbf{Conditional} & \textbf{Joint} \\ \hline
Pre-trained & Available & Scarce\\ \hline
$I(A,B)$ & Yes & Yes\\ \hline
$H(A)$ & Yes & Yes\\ \hline
$H(A\mid B)$ & Yes & Yes\\ \hline
$H(B)$ & No & Yes\\ \hline
$H(A,B)$ & No & Yes\\ \hline
Scalability (\# rvs) & Hard & Simple\\ \hline
\end{tabular}
\caption{Summary of our methods.}\label{tableMI}
\end{table}
\end{comment} 
In particular, given two random variables $A,B$, we consider two different classes of diffusion processes. In the first case, the diffusion model is asymmetric, and the random variable $B$ is only considered as a conditioning signal. As such, we learn the score associated to the random variable $A$ with or without a conditioning signal $B$. On the other hand, it is possible to define a diffusion model for the joint random variable $[A,B]$, see \Cref{sec:multitime}, which allows modelling the joint, the marginals and the conditional measures. %This approach requires learning the score of the joint random variable $[A,B]$.

The practical trade-off between the two families of approaches is simple: on the one hand, pre-trained conditional models are largely available, but are limited to only two random variables; on the other hand, joint models require an appropriate training procedure, but are more flexible and allow scaling beyond two random variables. \noteGF{We should kill the discussion about scaling.}

%\subsection{Conditional Diffusion models ($A\g B$)}\label{sec:conddiff}
%We here consider models that use both the unconditional $s^A_t(x)$ and the conditional $s^{A\g B}_t(x;y)$ score functions, where the notation indicates that we use the condition $B=y$. {\color{red} Typically, pretrained models for interesting applications are available ...}

A simple \gls{MI} estimator can be obtained considering \Cref{eq:mi_2}.% $\textsc{H}(A)-\textsc{H}(A\g B)$. 
The entropy of $A$ can be computed using \Cref{entropy_est}. Similarly, we can compute the conditional entropy $\textsc{H}(A\g B)$ using the equality $\textsc{H}(A\g B)=\int \textsc{H}(A\g B=y)\dd\mu^{B}(y)$, where the argument of the integral, $\textsc{H}(A\g B=y)$, can be again obtained using \Cref{entropy_est}. A second option is to leverage \Cref{eq:mi_1}. The two options correspond to estimating the \gls{MI} using either of the two: $-e(\mu^{A},\GaussM{\sigma})+\int e(\mu^{A\g B=y},\GaussM{\sigma})\dd\mu^{B}(y) $, or $ \int e(\mu^{A\g B=y},\mu^{A})\dd\mu^{B}(y)$. 
\begin{comment}
%\begin{footnotesize}
\begin{subequations}\label{condinfo1}
    \begin{multicols}{2}
        \begin{equation}
-e(\mu^{A},\GaussM{\sigma})+\int e(\mu^{A\g B=y},\GaussM{\sigma})\dd\mu^{B}(y) \label{condinfo1_1}
        \end{equation}%\break\hspace*{-3cm}
        \begin{equation}
            -\int e(\mu^{A\g B=y},\mu^{A})\dd\mu^{B}(y).   \label{condinfo1_2}
        \end{equation}
    \end{multicols}
\end{subequations}
%\end{footnotesize}
\end{comment}
\begin{comment}

%\hat{\textsc{I}}(A,B)=&
\begin{flalign}\label{condinfo1}
  -e(\mu^{A},\GaussM{\sigma})+\int e(\mu^{A\g B=y},\GaussM{\sigma})\dd\mu^{B}(y),\quad-\int e(\mu^{A\g B=y},\mu^{A})\dd\mu^{B}(y).
\end{flalign}
\end{comment}
{\color{red} Numerically, the second option should outperform the first one according to the cancelling of shared errors in the scores. We test this in the experimental section showing....}

%Being there no modelling of $\mu^{B}$, neither $\textsc{H}(B)$ nor $\textsc{H}(B\g A),\textsc{H}(A,B)$ are accessible when considering conditional models.

\subsection{Multitime}

Armed with the tools to describe multi-time diffusion processes, and the corresponding score functions, we can now proceed to determine the basic ingredients that allow computing the \gls{MI}, in its various formulations. Using multi-time score functions $s^{[A,B]}_{t,t}(x,y)$, the estimation of the joint entropy $\textsc{H}(A, B)$
is obtained with a straightforward application of \Cref{entropy_est}.
\begin{comment}
$e(\mu^{[A,B]},\GaussM{\sigma})$ as

\begin{flalign}
&\int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{A}(x_t\g x_0)\dd\nu_t^{B}(y_t\g y_0)\nonumber\\ &\norm{s^{[A,B]}_{t,t}(x_t,y_t)+
\frac{[x_t,y_t]^\top}{\exp(-2t)\sigma^2+1-\exp(-2t)} }^2\dd t.
\end{flalign}
\end{comment}
Similarly, the conditional entropy $\textsc{H}(A\g B)=\int \textsc{H}(A\g B=y)\dd\mu^{B}(y)$ can be computed using $s^{[A,B]}_{t,0}(x,y)$ to obtain the conditional score. Finally, the marginal entropy $\textsc{H}(A)$ can be computed using  $s^{[A,B]}_{t,\infty}(x,y)$. Notice that $\textsc{H}(B\g A),\textsc{H}(B)$ are similarly obtained by flipping the roles of $\alpha,\beta$. Given the above formulations of the joint, conditional and marginal entropy, it is now easy to compute the \gls{MI} according to \Cref{eq:mi_2,eq:mi_3,eq:mi_4}.

\begin{comment}
$e(\nu^{A\g B}_0,\GaussM{\sigma})$ as
\begin{flalign}
  &\int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[A]}(x_t\g x_0)\nonumber\\ &\norm{s^{[A,B]}_{t,0}(x_t,y_0)+
\frac{x_t}{\exp(-2t)\sigma^2+1-\exp(-2t)} }^2\dd t,
\end{flalign}
and similarly for $\textsc{H}(B\g A)$. 

Finally, the marginal entropy $\textsc{H}(A),\textsc{H}(B)$ can be obtained using $e(\mu^{A},\GaussM{\sigma})$ as \notePM{Double check me!}

\begin{flalign}
    & \int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[A]}(x_t\g x_0)\nonumber\\&\norm{s^{[A,B]}_{t,\infty}(x_t,y_0)+
\frac{x_t}{\exp(-2t)\sigma^2+1-\exp(-2t)} }^2\dd t. 
\end{flalign}
\end{comment}


Another strategy is to compute directly the \gls{MI} according to \Cref{eq:mi_1}. Then we can estimate $\KL{\mu^{[A,B]}}{\mu^{A}\mu^{B}}$ using $e(\mu^{[A,B]},\mu^{A}\mu^{B})$ given that all the necessary score functions are available. Alternatively, we can adopt \Cref{eq:mi_1}, where $\int \KL{\mu^{A\g B=y}}{\mu^{A}} \dd\mu^{B}(y)=\int e(\mu^{A\g B=y},\mu^{A})\dd\mu^{B}(y)$.% is estimated using the same strategy of \Cref{condinfo1_2}.

\begin{comment}

\begin{flalign}
 &\int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[A]}(x_t\g x_0)\dd\nu_t^{B}(y_t\g y_0)\nonumber\\&\norm{s^{[A,B]}_{t,t}(x_t,y_t)-\left[s^{[A,B]}_{t,\infty}(x_t,y_t),s^{[A,B]}_{\infty,t}(x_t,y_t)\right]^\top }^2\dd t.
\end{flalign}

Note that, since 
\begin{align*}
\KL{\mu^{[A,B]}}{\mu^{A}\mu^{B}} & = \E_{\mu^{B}}\left[\KL{\nu^{[A\g B]}}{\mu^{A}}\right]\\
                                 & =\E_{\mu^{A}}\left[\KL{\nu^{[B\g A]}}{\mu^{B}}\right],
\end{align*}
we can also estimate $\KL{\mu^{[A,B]}}{\mu^{A}\mu^{B}}$ as:

\begin{multline}
  \left[ \int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[A]}(x_t\g x_0) \right.\\
    \left. \norm{s^{[A,B]}_{t,0}(x_t,y_0)-s^{[A,B]}_{t,\infty}(x_t,y_0) }^2\dd t\right] = \\ 
  \left[\int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[B]}(y_t\g y_0) \right.\\
    \left. \norm{s^{[A,B]}_{0,y}(x_0,y_t)-s^{[A,B]}_{\infty,t}(x_0,y_t) }^2\dd t\right]  
\end{multline}

% \begin{flalign}
%  &\left[\int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[A]}(x_t\g x_0)\norm{s^{[A,B]}_{t,0}(x_t,y_0)-s^{[A,B]}_{t,\infty}(x_t,y_0) }^2\dd t\right]=\\
%  &\left[\int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[B]}(y_t\g y_0)\norm{s^{[A,B]}_{0,y}(x_0,y_t)-s^{[A,B]}_{\infty,t}(x_0,y_t) }^2\dd t\right]
% \end{flalign}
\end{comment}


==> mutual_information.tex <==
%All the applications described in the previous section could be spin-off works by themselves. In this paper, we want to focus specifically on the estimation of \textbf{mutual information}


The \gls{MI} between two random variables $A,B$ has several equivalent expressions

\begin{flalign}
    &\textsc{I}(A,B)=\KL{\nu^{[A,B]}_0}{\nu^{A}_0\nu^{B}_0}=\\&\textsc{H}(A)-\textsc{H}(A\g B)=\textsc{H}(B)-\textsc{H}(B\g A)=\\&\textsc{H}(A,B)-\textsc{H}(A\g B)-\textsc{H}(B\g A)=\\&\textsc{H}(A)+\textsc{H}(B)-\textsc{H}(A,B)
\end{flalign}
where $\nu^{[A,B]}_0$ is the measure corresponding to the joint random variable $[A,B]$. To leverage the same methodology we describe in \Cref{sec:diffusion} and apply it to the \gls{KL} formulation of \gls{MI}, it is sufficient to build a diffusion process corresponding to the joint measure $\nu^{[A,B]}_0$, with overall path measure $\mathbb{P}^{[A,B]}$, as follows

\begin{equation}\label{eq:diffsdesjoint}
    \begin{cases}
    \dd \left[X_t,Y_t\right]^\top =f_t[X_t,Y_t]^\top \dd t+ g_t\left[\dd W_t,\dd W'_t\right]^\top,\\
    [X_0,Y_0]^\top\sim \nu^{[A,B]}_0.
    \end{cases}
\end{equation}

Our goal here is to specify how it is possible to use score functions to estimate the mutual information $\textsc{I}(A,B)$. Different approaches either leverage pretrained diffusion models or require modification to the training schemes of diffusion models. In particular, we consider two different classes of diffusion models for the estimation of mutual information i) conditional and ii) joint. In the first case, the model is asymmetric in that the second random variable $B$ is always considered as a conditioning signal. In the case of images and text, for example, the random variable $A$ corresponds to images, while $B$ to text. In the conditional setting, what is modelled is the score of the variable $A$ with or without a conditioning signal $B$. What is \textbf{not} modelled is the score of the joint random variables $[A,B]$ nor of the variable $B$.

On the other hand, it is possible to construct diffusion models for the joint random variable $[A,B]$, modelling the joint, the marginals and the conditional measures.

In \Cref{tableMI} we report a schematic overview of pros and cons of the two choices. On the one hand, there is huge availability of pretrained conditional models, that can be used to compute the mutual information. Due to their structure, joint entropy and the marginal entropy of $B$ are unavailable. Moreover, when considering more than two random variables, their scalability is difficult. On the other hand, joint diffusion models are less common, but estimation of all the quantities is straightforward and they naturally scale to multiple modalities.

\begin{table}[ht]
\small
\centering
\begin{tabular}{|c|c|c|}
\hline
  & Conditional & Joint \\ \hline
Pretrained Av. & Very high & Scarce\\ \hline
$I(A,B)$ & Yes & Yes\\ \hline
$H(A)$ & Yes & Yes\\ \hline
$H(A\mid B)$ & Yes & Yes\\ \hline
$H(B)$ & No & Yes\\ \hline
$H(A,B)$ & No & Yes\\ \hline
Scalability (\# rvs) & Hard & Simple\\ \hline
\end{tabular}
\caption{MI estimators}\label{tableMI}
\end{table}

\begin{comment}
\begin{table}[ht]
\small
%\hspace*{-2cm}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
  & Pretrained Availability & $I(A,B)$ & $H(A)$ & $H(A\g B)$ & $H(B)$ & $H(A,B)$ & Scalability (\# rvs)\\ \hline
Conditional ($A\g B$) & Very high& Yes& Yes & Yes & No & No & Hard\\ \hline
%Joint (single-time) & Medium & Approx & Approx & Approx& Approx & Yes\\ \hline
Joint (multi-time) & Scarce & Yes & Yes & Yes & Yes & Yes & Simple\\
\hline
\end{tabular}
\caption{Example table with split row}\label{tableMI}
\end{table}
\end{comment}

\subsection{Conditional Diffusion models ($A\g B$)}
In this case the model learns the unconditional score $s^A_t(x)$ and the conditional score $s^{A\g B}_t(x;y)$, where this new notation indicates that we condition $B=y$.


A first trivial estimator of the mutual information can then be obtained considering $\textsc{H}(A)-\textsc{H}(A\g B)$. The entropy of $A$ can be computed using \Cref{entropy_est}. Similarly, we can compute the conditional entropy $\textsc{H}(A\g B)$ using the equality $\textsc{H}(A\g B)=\int \textsc{H}(A\g B=y)\dd\nu^B_0(y)$, where the inner values of the integral, $\textsc{H}(A\g B=y)$, are computed once again using \Cref{entropy_est}. Then, the mutual information $\textsc{I}(A,B)$ is computed as
%\begin{equation}\label{condentropy_est}
%   \textsc{H}(A\g B)=\int \textsc{H}(A\g B=y)\dd\nu^B_0(y) = -\int e_T(\nu^{A\g B=y}_0,\mathcal{N}(0,\sigma^2))\dd\nu^B_0(y) +\frac{1}{2}\log(2\pi \sigma^2).
%\end{equation}
\begin{flalign}\label{condinfo1}
  &-e_T(\nu^A_0,\mathcal{N}(0,\sigma^2))+\int e_T(\nu^{A\g B=y}_0,\GaussM{0,\sigma^2})\dd\nu^B_0(y) %\left(-e_T(\nu^A_0,\mathcal{N}(0,\sigma^2))+\frac{1}{2}\log(2\pi \sigma^2)\right) -\left( -\int e_T(\nu^{A\g B=y}_0,\mathcal{N}(0,\sigma^2))\dd\nu^B_0(y) +\frac{1}{2}\log(2\pi \sigma^2)\right)=\nonumber\\&-e_T(\nu^A_0,\mathcal{N}(0,\sigma^2))+\int e_T(\nu^{A\g B=y}_0,\mathcal{N}(0,\sigma^2))\dd\nu^B_0(y)
\end{flalign}
%This estimator is valid for \textit{any} $\sigma$ (different choices different tradeoffs?)

A second option is to leverage the equality $ \textsc{I}(A,B)=\int \KL{\nu^{A\g B=y}}{\nu^{A}} \dd\nu^B_0(y)$ to obtain 
\begin{equation}\label{condinfo2}
  \textsc{I}(A,B)=\int e_T(\nu^{A\g B=y}_0,\nu^A_0)\dd\nu^B_0(y)
\end{equation}

Effectively, the two estimators \Cref{condinfo1,condinfo2} correspond to 

\begin{flalign}
 &\frac{T}{2}\E\left[g^2_t\left(-\norm{{s}^{A}_t(X_t)+\chi^{-1}_tX_t}^2+\norm{{s}^{A\g B=Y_0}_t(X_t) +\chi^{-1}_tX_t}^2\right)\right],\\ &\frac{T}{2}\E\left[g^2_t\norm{{s}^{A}_t(X_t)-{s}^{A\g B=Y_0}_t(X_t) }^2\right],   
\end{flalign}
where the expected value has to be understood as
$E_{   [X_0,Y_0]\sim\nu_0^{[A,B]},t\sim\mathcal{U}(0,T),X_t\sim\nu_t^{A\g X_0}}
$. {\color{red} The bias should self cancel in option \#2, due to the cancelling of common errors}

%Being there no modelling of $\nu^B$, neither $\textsc{H}(B)$ nor $\textsc{H}(B\g A),\textsc{H}(A,B)$ are accessible when considering conditional models.



\subsection{Multitime diffusion models}


Being there no modelling of $\nu^B$, neither $\textsc{H}(B)$ nor $\textsc{H}(B\g A),\textsc{H}(A,B)$ are accessible when considering conditional models. To remedy on this, in this Section we present an extension of diffusion models which is amenable to learn the score of the joint, marginals and conditional measures.

The joint measure score $s^{[A,B]}_t(x,y)$ is the one corresponding to the process in \Cref{eq:diffsdesjoint}.
With a slight abuse of notation, we introduce the concept of \textit{multi-time} for the score functions.
The joint score is in this context indicated with $s^{[A,B]}_{t,t}(x,y)$, i.e. with a double (equal) argument $t$. As explained hereafter, this new notation choice allows to efficiently describe conditional and marginal scores. Under the modified notation, the conditional score 
%\begin{equation}
%    s^{A\g B}_t(x;y)=\nabla_x\log \left(\tilde\nu^{A\g B=y}_t(x)\right)=\nabla_x\log \left(\tilde\nu^{A\g B=y}_t(x)\tilde\nu^{B}_0(y)\right)
%\end{equation} 
\begin{equation}
    s^{A\g B}_t(x;y)=\nabla_x\log \left(\tilde\nu^{A\g B=y}_t(x)\tilde\nu^{B}_0(y)\right)
\end{equation}
is replaced by the $x-$part of $s^{[A,B]}_{t,0}(x,y)$. This can be understood considering that the conditional score corresponds to the $x-$part of the score of the \textit{modified} diffusion process 

\begin{equation}\label{eq:diffsdesjoint}
    \begin{cases}
    \dd \left[X_t,Y_t\right]^\top =f_t[X_t,{\color{red} 0\times}Y_t]^\top \dd t+ g_t\left[\dd W_t,{\color{red} 0\times}\dd W'_t\right]^\top,\\
    [X_0,Y_0]^\top\sim \nu^{[A,B]}_0.
    \end{cases}
\end{equation}
Effectively, the modification forces the value $Y_t=Y_0$ throughout all the stochastic evolution.

Similarly, the marginal score $s^{A}_{t}(x)$ is substituted by the $x-$part of $s^{[A,B]}_{t,\infty}(x,y)$, considering the \textit{modified} diffusion process 
\begin{equation}\label{eq:diffsdesjoint}
    \begin{cases}
    \dd \left[X_t,Y_t\right]^\top =f_t[X_t,{\color{red} \infty\times}Y_t]^\top \dd t+ g_t\left[\dd W_t,{\color{red} \infty\times}\dd W'_t\right]^\top,\\
    [X_0,Y_0]^\top\sim \nu^{[A,B]}_0.
    \end{cases}
\end{equation}
where the $\infty$ term (abuse of notation) drives immediately the $y-$ part of the process into its uninformative, decorrelated from initial conditions, steady state.
Notice that while $s^{[A,B]}_{t,t}(x,y)\in \mathbb{R}^{2N}$, instead $s^{[A,B]}_{t,0}(x,y),s^{[A,B]}_{t,\infty}(x,y)\in \mathbb{R}^{N}$ as they correspond to the $x-$parts of the modified diffusion processes. Similarly, $s^{[A,B]}_{0,t}(x,y),s^{[A,B]}_{\infty,t}(x,y)$ corresponds to the $y-$parts of modified processes.


When considering multi-time models $s^{[A,B]}_{t,t}(x,y)$, estimation of the joint entropy $\textsc{H}(A, B)=-e_T(\nu^{[A,B]}_0,\GaussM{0,\sigma^2})+\frac{1}{2}\log(2\pi \sigma^2)$ is obtained estimating $e_T(\nu^{[A,B]}_0,\GaussM{0,\sigma^2})$ as

\begin{flalign}
&\int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{A}(x_t\g x_0)\dd\nu_t^{B}(y_t\g y_0)\nonumber\\ &\norm{s^{[A,B]}_{t,t}(x_t,y_t)+
\frac{[x_t,y_t]^\top}{\exp(-2t)\sigma^2+1-\exp(-2t)} }^2\dd t
\end{flalign}
The conditional entropy $\textsc{H}(A\g B)$ can similarly be computed using $e_T(\nu^{A\g B}_0,\GaussM{0,\sigma^2})$
\begin{flalign}
  &\int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[A]}(x_t\g x_0)\nonumber\\ &\norm{s^{[A,B]}_{t,0}(x_t,y_0)+
\frac{x_t}{\exp(-2t)\sigma^2+1-\exp(-2t)} }^2\dd t,
\end{flalign}
and similarly for $\textsc{H}(B\g A)$. Finally, marginal entropies $\textsc{H}(A),\textsc{H}(B)$ can be obtained considering

\begin{flalign}
    & \int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[A]}(x_t\g x_0)\nonumber\\&\norm{s^{[A,B]}_{t,\infty}(x_t,y_0)+
\frac{x_t}{\exp(-2t)\sigma^2+1-\exp(-2t)} }^2\dd t 
\end{flalign}

To compute the mutual information, we can use the conditional entropies, leveraging $ \textsc{I}(A,B)=\textsc{H}(A,B)-\textsc{H}(A\g B)-\textsc{H}(B\g A)$. Alternatively it is possible to compute the couples $\textsc{H}(A),\textsc{H}(A\g B)$ or $\textsc{H}(B),\textsc{H}(B\g A)$. Yet an other strategy is to directly compute  $\KL{\nu^{[A,B]}}{\nu^{A}\nu^{B}}$ as

\begin{flalign}
 &\int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[A]}(x_t\g x_0)\dd\nu_t^{B}(y_t\g y_0)\nonumber\\&\norm{s^{[A,B]}_{t,t}(x_t,y_t)-\left[s^{[A,B]}_{t,\infty}(x_t,y_t),s^{[A,B]}_{\infty,t}(x_t,y_t)\right]^\top }^2\dd t
\end{flalign}
or, since $\KL{\nu^{[A,B]}}{\nu^{A}\nu^{B}}=\E_{\nu^B}\left[\KL{\nu^{[A\g B]}}{\nu^{A}}\right]=\E_{\nu^A}\left[\KL{\nu^{[B\g A]}}{\nu^{B}}\right]$,

\begin{flalign}
 &\left[\int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[A]}(x_t\g x_0)\norm{s^{[A,B]}_{t,0}(x_t,y_0)-s^{[A,B]}_{t,\infty}(x_t,y_0) }^2\dd t\right]=\\&\left[\int \dd\nu_0^{[A,B]}(x_0,y_0)\int\limits_0^T\int\dd\nu_t^{[B]}(y_t\g y_0)\norm{s^{[A,B]}_{0,y}(x_0,y_t)-s^{[A,B]}_{\infty,t}(x_0,y_t) }^2\dd t\right]
\end{flalign}



\begin{comment}
Before proceeding, a couple of useful equalities:

\begin{flalign}
  &\int \nabla_x \log \nu_t^{[A,B]}(x,y) \dd\nu_t^{B\g A}(y\g x)=\int \nabla_x \log \nu_t^{A\g B}(x\g y) \dd\nu_t^{B\g A}(y\g x)=\int \nabla_x \nu_t^{A\g B}(x\g y) \frac{\dd\nu_t^{B\g A}(y\g x)}{\nu_t^{A\g B}(x\g y)}= \nonumber\\&=\int \nabla_x \nu_t^{A\g B}(x\g y) \frac{\nu_t^{B\g A}(y\g x)\dd y}{\nu_t^{A\g B}(x\g y)}=\int \nabla_x \nu_t^{A\g B}(x\g y) \frac{\nu_t^{B\g A}(y\g x)\nu^B_t(y)\dd y}{\nu_t^{B\g A}(y\g x)\nu^A_t(x)}=\nonumber\\&\int \nabla_x \nu_t^{A\g B}(x\g y) \frac{\nu^B_t(y)\dd y}{\nu^A_t(x)}=\nabla_x \frac{\int \nu_t^{A\g B}(x\g y)\nu^B_t(y)\dd y}{\nu^A_t(x)}=\nabla_x \log \nu_t^A(x)
\end{flalign}

\begin{flalign}
    &\dd\nu_t^{B\g A}(y\g x)=\int \dd\nu_t^{B\g A}(y,x_0\g x)\dd x_0=\int \dd\nu_t^{B\g A}(y\g x_0)\dd\nu(x_0\g x)\dd x_0
\end{flalign}

\begin{flalign}
    &\dd\nu_t^{B\g A}(y\g x_0)=\int \dd\nu_t^{B\g A}(y,x_t\g x_0)\dd x_t=\int \frac{\dd\nu(x_0\g y,x_t)}{\dd\nu(x_0)}\dd\nu(y,x_t)\dd x_t
\end{flalign}

\subsubsection{Single time}
In this scenario a "classical" diffusion model is trained simultaneously on the joint random variable $[A,B]$. Consequently the joint entropy $\textsc{H}(A,B)$ is easily computed, as the joint score $\nabla\log \nu^{[A,B]}_t(x,y)$ is explicitly modelled.

To compute the mutual information, it is necessary to compute the conditional entropies ($\textsc{H}(A\g B)\textsc{H}(B\g A)$), leveraging $ \textsc{I}(A,B)=\textsc{H}(A,B)-\textsc{H}(A\g B)-\textsc{H}(B\g A)$. Alternatively it is possible to estimate the couples $\textsc{H}(A),\textsc{H}(A\g B)$ or $\textsc{H}(B),\textsc{H}(B\g A)$. Finally, yet an other strategy is to compute  $\KL{\nu^{[A.B]}}{\nu^{A}\nu^{B}}$.
\end{comment}




==> mutual_information_v2.tex <==
%\noteGF{I think the biggest problem of this Section is that we present 10 different ways of computing the MI, but other than a "we tested and this work better" we have no clue why certain parametrizations are better than others.}

In this work, we are interested in estimating the \gls{MI} between two random variables $A,B$. Consequently, we need to define the joint, conditional and marginal measures. We consider the first random variable $A$ in $\mathbb{R}^N$ to have marginal measure $\mu^{A}$. Similarly, we indicate the marginal measure of the second random variable $B$ with $\mu^{B}$. The joint measure of the two random variables $C\defeq[ A,B]$, which is defined in $\mathbb{R}^{2N}$, is indicated with $\mu^{C}$. What remains to be specified are the conditional measures of the first variable given a particular value of the second $A\g B= y$, shortened with $A_y$, that we indicate with the measure $\mu^{A_y}$, and the conditional measure of the second given a particular value of the first, $B\g A= x$, shortened with $B_x$, and indicated with $\mu^{B_x}$. This choice of notation, along with Bayes theorem, implies the following set of equivalences: $\dd\mu^{C}(x,y)=\dd\mu^{A_y}(x)\dd\mu^{B}(y)=\dd\mu^{B_x}(y)\dd\mu^{A}(x)$ and $\mu^{A}=\int \mu^{A_y}\dd\mu^{B}(y),\mu^{B}=\int\mu^{B_x}\dd\mu^{A}(x)$.

%{\color{red} We conclude our introduction with an important clarification on the \textbf{notation}. Every object, when considering a different random variable $B$ from which initial conditions are drawn, inherits the same convention with the variable $B$ in place of $A$. To clarify, the equivalent of \Cref{eq:diffsdes} with a different random variable $B$ is a process that starts from initial conditions $\mu^B$, with an overall path measure $\mathbb{P}^{B}$, pushforward $\nu^B_t$, path reversed measure $\hat{\mathbb{P}}^{B}$ and score function $s^{B}_t(x)$. As exemplified hereafter, the same holds when considering jointly random variables $C$, or a random variable conditionally on a particular value of a second one, $A_y$.}

As a starting point, we recognize that the \gls{MI} between two random variables $A,B$ has several equivalent expressions, among which \Cref{eq:mi_1,eq:mi_2,eq:mi_3}. On the left hand side of these expressions we report well-known formulations for the \gls{MI}, $\textsc{I}(A,B)$, while on the right hand side we express them using the estimators we introduce in this work, where equality is assumed to be valid up to the errors described in \Cref{sec:kl_deriv}. {\color{red}Complete details and derivations are provided in Appendix.}


\begin{footnotesize}
%\begin{alignLetter}
\begin{align}
    %\KL{\mu^{C}}{\mu^{A}\mu^{B}}\simeq &e(\mu^{C},\mu^{A}\mu^{B}) \label{eq:mi_0}\\
    \textsc{H}(A)-\textsc{H}(A\g B)\simeq & -e(\mu^{A},\GaussM{\sigma})+\int e(\mu^{A_y},\GaussM{\sigma})\dd\mu^{B}(y)\label{eq:mi_2},\\
    \int \KL{\mu^{A_y}}{\mu^{A}} \dd\mu^{B}(y)\simeq & \int e(\mu^{A_y},\mu^{A})\dd\mu^{B}(y) \label{eq:mi_1},\\
    \textsc{H}(C)-\textsc{H}(A\g B)-\textsc{H}(B\g A)\simeq & -e(\mu^{C},\GaussM{\sigma})+\int e(\mu^{A_y},\GaussM{\sigma})\dd\mu^{B}(y)+\int e(\mu^{B_x},\GaussM{\sigma})\dd\mu^{A}(x).\label{eq:mi_3}
    %\simeq &\E_{\mathbb{P}^{\mu^{C}}}\left[\int\limits_0^T\frac{g^2_{t}}{2} \left[\norm{{s}^{\mu^{C}}_{t}([X_t,Y_t])-[s^{\mu^{A_{Y_0}}}_{t}(X_t),s^{\mu^{B_{X_0}}}_{t}(Y_t)] }^2\right]\dd t\right] \label{eq:mi_3inner}
    %\textsc{H}(A)+\textsc{H}(B)-\textsc{H}(C)\simeq &-e(\mu^{A},\GaussM{\sigma})-e(\mu^{B},\GaussM{\sigma}) +e(\mu^{C},\GaussM{\sigma})\label{eq:mi_4}
\end{align}
\end{footnotesize}

\begin{comment}
\begin{alignLetter}
    \KL{\mu^{C}}{\mu^{A}\mu^{B}}=&e(\mu^{C},\mu^{A}\mu^{B})= \label{eq:mi_0}\\
    \E_{\mu^{B}}\left[\KL{\mu^{A_y}}{\mu^{A}}\right]=& \E_{\mu^{B}}\left[e(\mu^{A_y},\mu^{A})\right]=\label{eq:mi_1}\\
    \textsc{H}(A)-\textsc{H}(A\g B)=& -e(\mu^{A},\GaussM{\sigma})+\E_{\mu^{B}}\left[e(\mu^{A_y},\GaussM{\sigma})\right]\label{eq:mi_2}\\
    \textsc{H}(A,B)-\textsc{H}(A\g B)-\textsc{H}(B\g A)=& -e(\mu^{C},\GaussM{\sigma})+\E_{\mu^{B}}\left[e(\mu^{A_y},\GaussM{\sigma})\right]+\int e(\mu^{B_x},\GaussM{\sigma})\dd\mu^{A}(x)\label{eq:mi_3}\\
    \textsc{H}(A)+\textsc{H}(B)-\textsc{H}(A,B)=&-e(\mu^{A},\GaussM{\sigma})-e(\mu^{B},\GaussM{\sigma}) +e(\mu^{C},\GaussM{\sigma})\label{eq:mi_4}
\end{alignLetter}
\end{comment}
%Then, we present several alternatives to leverage the methodology introduced in \Cref{sec:diffusion}, and apply it to compute the \gls{MI} according to its various formulations. 
% Our methods either capitalize on pre-trained diffusion models, or require training from scratch, and come with a variety of properties. %, as summarized in \Cref{tableMI}.
\begin{comment}
\begin{table}[ht]
\small
\centering
\begin{tabular}{|c|c|c|}
\hline
  & \textbf{Conditional} & \textbf{Joint} \\ \hline
Pre-trained & Available & Scarce\\ \hline
$I(A,B)$ & Yes & Yes\\ \hline
$H(A)$ & Yes & Yes\\ \hline
$H(A\mid B)$ & Yes & Yes\\ \hline
$H(B)$ & No & Yes\\ \hline
$H(A,B)$ & No & Yes\\ \hline
Scalability (\# rvs) & Hard & Simple\\ \hline
\end{tabular}
\caption{Summary of our methods.}\label{tableMI}
\end{table}
\end{comment} 

% We are now ready to describe our new \gls{MI} estimator, which we call \gls{MINDE}. Note that the methodology discussed in \Cref{sec:kl_deriv} induces a \textit{family} of techniques to estimate \gls{MI}. An appropriate choice depends on several factors, including the availability of pre-trained models. First, we consider estimation of the \gls{MI} using \textit{standard} diffusion processes. Then, in \Cref{sec:multitime} we consider a new class of diffusion processes that have been recently introduced in the literature \citep{bao2023transformer, bounoua2023multimodal}, which allows to generalize our proposed methodology.

% Our methods either capitalize on pre-trained diffusion models, or require training from scratch, and come with a variety of properties.
% In particular, given two random variables $A,B$, we consider two classes of diffusion processes. In the first case, the diffusion model is asymmetric, and the random variable $B$ is only considered as a conditioning signal. As such, we learn the score associated to the random variable $A$ with or without a conditioning signal $B$. On the other hand, it is possible to define a diffusion model for the joint random variable $C$, see \Cref{sec:multitime}, which allows modelling the joint, the marginals and the conditional measures. %This approach requires learning the score of the joint random variable $C$.

We are now ready to describe our new \gls{MI} estimator, which we call \gls{MINDE}. Note that the methodology discussed in \Cref{sec:kl_deriv} induces a \textit{family} of techniques to estimate \gls{MI}. 
% Indeed, our methods either capitalize on pre-trained diffusion models, or require training from scratch, and come with a variety of properties.
In particular, given two random variables $A,B$, we consider two classes of diffusion processes. In the first case, the diffusion model is asymmetric, and the random variable $B$ is only considered as a conditioning signal. As such, we learn the score associated to the random variable $A$ with or without a conditioning signal $B$. On the other hand, it is possible to define a diffusion model for the joint random variable $C$, which allows modelling the joint and the conditional measures. %, as described in \Cref{sec:multitime}.
% , we consider a new class of diffusion processes that have been recently introduced in the literature \citep{bao2023transformer, bounoua2023multimodal}.
An appropriate choice between the conditional and joint modeling approaches depends on several factors, including the availability of pre-trained models. 

 %This approach requires learning the score of the joint random variable $C$.


\paragraph{Conditional Diffusion Models.} We start considering conditional models. 
A simple \gls{MI} estimator can be obtained considering \Cref{eq:mi_2}. % $\textsc{H}(A)-\textsc{H}(A\g B)$. 
The entropy of $A$ can be estimated using \Cref{entropy_est}.
% as $\frac{N}{2}\left(\log(2\pi \sigma^2)-\left(\log{(\chi_{T}})-1+\nicefrac{1}{\chi_{T}}\right)\right)+\frac{\E_{\mu^A}\left[X_0^2\right]}{2\sigma^2}-e(\mu^A,\GaussM{\sigma})$. 
Similarly, we can estimate the conditional entropy $\textsc{H}(A\g B)$ using the equality $\textsc{H}(A\g B)=\int \textsc{H}(A_y)\dd\mu^{B}(y)$, where the argument of the integral, $\textsc{H}(A_y)$, can be again obtained using \Cref{entropy_est}. Notice, that since $\E_{\mu^B(y)}\E_{\mu^{A_y}}\left[X_0^2\right]=\E_{\mu^A}\left[X_0^2\right]$, when substracting the estimators of $\textsc{H}(A)$ and $\textsc{H}(A\g B)$, all the terms but the estimator functions $e(\cdot)$ cancels out, leading to the equality in \Cref{eq:mi_2}. A second option is to simply use \Cref{eq:mi_1} and leverage \Cref{eq:estimator}. %{\color{red} !!In \Cref{sec:miperspective} we showcase the application of conditional models, using a pre-trained text-to-image generative model. For more general settings, e.g. when pre-trained models are not available, the method we present later is a preferable choice, and we use it in our extensive evaluation presented in \Cref{sec:experiments}.}

%\notePM{Remember to say why is preferable, end of sec 4.1.}

% The two options correspond to estimating the \gls{MI} using either of the two: $-e(\mu^{A},\GaussM{\sigma})+\int e(\mu^{A_y},\GaussM{\sigma})\dd\mu^{B}(y) $, or $ \int e(\mu^{A_y},\mu^{A})\dd\mu^{B}(y)$. 
\begin{comment}
%\begin{footnotesize}
\begin{subequations}\label{condinfo1}
    \begin{multicols}{2}
        \begin{equation}
-e(\mu^{A},\GaussM{\sigma})+\int e(\mu^{A_y},\GaussM{\sigma})\dd\mu^{B}(y) \label{condinfo1_1}
        \end{equation}%\break\hspace*{-3cm}
        \begin{equation}
            -\int e(\mu^{A_y},\mu^{A})\dd\mu^{B}(y).   \label{condinfo1_2}
        \end{equation}
    \end{multicols}
\end{subequations}
%\end{footnotesize}
\end{comment}
\begin{comment}

%\hat{\textsc{I}}(A,B)=&
\begin{flalign}\label{condinfo1}
  -e(\mu^{A},\GaussM{\sigma})+\int e(\mu^{A_y},\GaussM{\sigma})\dd\mu^{B}(y),\quad-\int e(\mu^{A_y},\mu^{A})\dd\mu^{B}(y).
\end{flalign}
\end{comment}
%{\color{red} Numerically, the second option should outperform the first one according to the cancelling of shared errors in the scores. We test this in the experimental section showing....}

\input{MI/multitime_diff}



Armed with the tools to define masked diffusion processes, and the corresponding score function, we now describe the basic ingredients that allow estimation of the \gls{MI}, according to various formulations. Using the joint score function $s^{\mu^{C}}_{t}([x,y])$, the estimation of the joint entropy $\textsc{H}(A, B)$ can be obtained with a straightforward application of \Cref{entropy_est}. Similarly, the conditional entropy $\textsc{H}(A\g B)=\int \textsc{H}(A_y)\dd\mu^{B}(y)$ can be computed using $s^{\mu^{A_y}}_{t}(x)$ to obtain the conditional score. Notice that $\textsc{H}(B\g A)$ is similarly obtained. Given the above formulations of the joint and conditional entropy, it is now easy to compute the \gls{MI} according to \Cref{eq:mi_3}, where we notice that, similarly to what discussed for conditional models, many of the terms in the different entropy estimations cancel out. 

Finally, it is worth to notice that it is possible to derive (proof in Appendix) yet an other equality for the \gls{MI}: 
\begin{equation}\label{eq:mi_3inner}
    \textsc{I}(A,B)\simeq\E_{\mathbb{P}^{\mu^{C}}}\left[\int\limits_0^T\frac{g^2_{t}}{2} \left[\norm{{\tilde s}^{\mu^{C}}_{t}([X_t,Y_t])-[\tilde s^{\mu^{A_{Y_0}}}_{t}(X_t),\tilde s^{\mu^{B_{X_0}}}_{t}(Y_t)] }^2\right]\dd t\right]. 
\end{equation}
Interestingly, this formulation allows to get rid of the parameter $\sigma$ of the entropies estimators. Similarly to the \gls{MINDE} conditional variant which shares this property (\Cref{eq:mi_2})Interestingly, the .. \noteGF{We need full results to comment!}
. %Another strategy is to compute directly the \gls{MI} according to \Cref{eq:mi_1}. Then we can estimate $\KL{\mu^{C}}{\mu^{A}\mu^{B}}$ using $e(\mu^{C},\mu^{A}\mu^{B})$ given that all the necessary score functions are available. Alternatively, we can adopt \Cref{eq:mi_1}, where $\int \KL{\mu^{A_y}}{\mu^{A}} \dd\mu^{B}(y)=\int e(\mu^{A_y},\mu^{A})\dd\mu^{B}(y)$.% is estimated using the same strategy of \Cref{condinfo1_2}.



%The practical trade-off between the two families of approaches is simple: on the one hand, pre-trained conditional models are largely available, but are limited to only two random variables; on the other hand, joint models require an appropriate training procedure, but are more flexible and allow scaling beyond two random variables. \noteGF{We should kill the discussion about scaling.}

%\subsection{Conditional Diffusion models ($A\g B$)}\label{sec:conddiff}
%We here consider models that use both the unconditional $s^A_t(x)$ and the conditional $s^{A\g B}_t(x;y)$ score functions, where the notation indicates that we use the condition $B=y$. {\color{red} Typically, pretrained models for interesting applications are available ...}




%Being there no modelling of $\mu^{B}$, neither $\textsc{H}(B)$ nor $\textsc{H}(B\g A),\textsc{H}(A,B)$ are accessible when considering conditional models.



%\subsection{Practical considerations}
%Difference inside vs difference outside...



==> tables/100k_full.tex <==
\renewcommand{\tabcolsep}{0.0pt}

\begin{table}[H]
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule

GT & 0.2 & 0.4 & 0.3 & 0.4 & 0.4 & 0.4 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 0.3 & 1.0 & 1.3 & 1.0 & 0.4 & 1.0 & 0.6 & 1.6 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.2 & 0.4 & 0.2 & 0.3 & 0.2 & 0.4 & 0.3 & 0.4 & 1.7 & 0.3 & 0.4 \\
\midrule
%mt\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D4DDE9}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{AFC4DD}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\textbf{ \gls{MINDE}--j ($\sigma=1$)} \ & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D4DDE9}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{EED3DB}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{AFC4DD}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D4DDE9}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%mt\_minde\_imp\_s
\textbf{ \gls{MINDE}--j}  & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{AFC4DD}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D4DDE9}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%c\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\textbf{ \gls{MINDE}--c ($\sigma=1$)} & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%c\_minde\_imp
%\textbf{ \gls{MINDE}--c ($\sigma=1$)}& {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\


%c\_minde\_imp\_s 
%\textbf{ \gls{MINDE}--c}& {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\textbf{ \gls{MINDE}--c} & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\midrule
MINE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{DB6185}} 0.6 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.1 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{D53D69}} -0.6 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E188A2}} 0.1 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
KSG & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{E188A2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{DB6185}} 0.6 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.1 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
LNN & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{4479BB}} 0.9 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.4 & {\cellcolor[HTML]{8CABD2}} 1.3 & {\cellcolor[HTML]{8CABD2}} 0.6 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 6.8 & {\cellcolor[HTML]{4479BB}} 33.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.4 & {\cellcolor[HTML]{4479BB}} 7.2 & {\cellcolor[HTML]{DB6185}} -0.2 & {\cellcolor[HTML]{D53D69}} -0.6 & {\cellcolor[HTML]{8CABD2}} 0.5 & {\cellcolor[HTML]{4479BB}} 1.2 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 5.5 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{E7ADBE}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
CCA & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{E188A2}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{AFC4DD}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{D4DDE9}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{E188A2}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{EED3DB}} 1.6 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
\midrule
dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=0.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=0.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\

\bottomrule
\end{tabular}

\caption{Mean MI estimates over 10 seeds using N = 10000 samples compared each against the ground-truth. Color indicates relative
negative bias (red) and positive bias (blue). Our method and all neural estimators were trained with 100k training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
\notePM{Explain color coding?}
}
\label{tab:benchmark}
\end{table}


==> tables/100k_full_std.tex <==
\renewcommand{\tabcolsep}{.0pt}

\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
% mt\_minde & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{9AB4D6}} .26 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 \\
\textbf{ \gls{MINDE}--j ($\sigma=1$)}  & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 \\
% mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{AFC4DD}} .20 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 \\
\textbf{ \gls{MINDE}--j} & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
% c\_minde & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{BFCEE2}} .16 & {\cellcolor[HTML]{BFCEE2}} .16 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
\textbf{ \gls{MINDE}--c ($\sigma=1$)} & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
% c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{BFCEE2}} .16 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 \\
\textbf{ \gls{MINDE}--c} & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 \\
\midrule
MINE & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 \\
D-V & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{4479BB}} 2.22 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 \\
KSG & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
LNN & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{B3C6DF}} .19 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{4479BB}} .50 & {\cellcolor[HTML]{B6C8DF}} .18 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
CCA & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{4479BB}} .61 & {\cellcolor[HTML]{4479BB}} .76 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{B3C6DF}} .19 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 
\\ DoE(Gaussian) & {\cellcolor[HTML]{E2E7EE}}.06 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{E9ECF0}}.04 & {\cellcolor[HTML]{D4DDE9}}.10 & {\cellcolor[HTML]{E9ECF0}}.04 & {\cellcolor[HTML]{E9ECF0}}.04 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{E9ECF0}}.04 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{E6EAEF}}.05 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{D4DDE9}}.10 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{E6EAEF}}.05 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{9AB4D6}}.26 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{DFE5ED}}.07 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{F2F2F2}}.01 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{DFE5ED}}.07 & {\cellcolor[HTML]{E9ECF0}}.04 & {\cellcolor[HTML]{EDEFF1}}.03 & & & {\cellcolor[HTML]{4479BB}} 1.05 & {\cellcolor[HTML]{4479BB}}.80 & {\cellcolor[HTML]{D4DDE9}}.10 & {\cellcolor[HTML]{4479BB}} 1.90 & {\cellcolor[HTML]{C1D0E3}}.15 & {\cellcolor[HTML]{DBE2EB}}.08 & {\cellcolor[HTML]{D4DDE9}}.10 & {\cellcolor[HTML]{F0F1F2}}.02 & \\
DoE(Logistic) & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{E2E7EE}}.06 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{D7DFEA}}.09 & {\cellcolor[HTML]{F2F2F2}}.01 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{F2F2F2}}.01 & {\cellcolor[HTML]{E9ECF0}}.04 & {\cellcolor[HTML]{C6D3E5}}.14 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{E9ECF0}}.04 & {\cellcolor[HTML]{E9ECF0}}.04 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{F2F2F2}}.01 & {\cellcolor[HTML]{F0F1F2}}.02 & {\cellcolor[HTML]{E2E7EE}}.06 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{4479BB}} 1.32 & {\cellcolor[HTML]{4479BB}} 1.42 & {\cellcolor[HTML]{E2E7EE}}.06 & {\cellcolor[HTML]{DFE5ED}}.07 & {\cellcolor[HTML]{E9ECF0}}.04 & {\cellcolor[HTML]{D0DAE8}}.11 & {\cellcolor[HTML]{DFE5ED}}.07 & {\cellcolor[HTML]{E9ECF0}}.04 & {\cellcolor[HTML]{EDEFF1}}.03 & {\cellcolor[HTML]{F0F1F2}}.02 &   \\




\\dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Standard deviation results over 10 seeds using N = 10000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 100k training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}
\label{std_100k}
\end{table}






==> tables/100k_nobasic.tex <==
\renewcommand{\tabcolsep}{0.0pt}

\begin{table}[H]
\vspace*{-0cm}
\tiny

\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule

GT & 0.2 & 0.4 & 0.3 & 0.4 & 0.4 & 0.4 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 0.3 & 1.0 & 1.3 & 1.0 & 0.4 & 1.0 & 0.6 & 1.6 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.2 & 0.4 & 0.2 & 0.3 & 0.2 & 0.4 & 0.3 & 0.4 & 1.7 & 0.3 & 0.4 \\
\midrule
%mt\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D4DDE9}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{AFC4DD}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\textbf{\gls{MINDE}--\textsc{j} ($\sigma=1$)} \ & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D4DDE9}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{EED3DB}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{AFC4DD}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D4DDE9}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%mt\_minde\_imp\_s
\textbf{\gls{MINDE}--\textsc{j}}  & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{AFC4DD}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D4DDE9}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%c\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\textbf{\gls{MINDE}--\textsc{c} ($\sigma=1$)} & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%c\_minde\_imp
%\textbf{ \gls{MINDE}--c ($\sigma=1$)}& {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\


%c\_minde\_imp\_s 
%\textbf{ \gls{MINDE}--c}& {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\textbf{\gls{MINDE}--\textsc{c}} & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\midrule
MINE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{DB6185}} 0.6 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.1 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{E7ADBE}} 0.0 & {\cellcolor[HTML]{D53D69}} -0.6 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E188A2}} 0.1 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%KSG & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{E188A2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{DB6185}} 0.6 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.1 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%LNN & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{4479BB}} 0.9 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.4 & {\cellcolor[HTML]{8CABD2}} 1.3 & {\cellcolor[HTML]{8CABD2}} 0.6 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 6.8 & {\cellcolor[HTML]{4479BB}} 33.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.4 & {\cellcolor[HTML]{4479BB}} 7.2 & {\cellcolor[HTML]{DB6185}} -0.2 & {\cellcolor[HTML]{D53D69}} -0.6 & {\cellcolor[HTML]{8CABD2}} 0.5 & {\cellcolor[HTML]{4479BB}} 1.2 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 5.5 & {\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{E7ADBE}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
\midrule
 & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=0.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=0.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\

\bottomrule
\end{tabular}}

\caption{Mean MI estimates over 10 seeds using N = 10k test samples against ground truth (GT). Color indicates relative
negative (red) and positive bias (blue). All methods were trained with 100k samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}
\label{tab:benchmark}

\end{table}


==> tables/10k_full.tex <==
\renewcommand{\tabcolsep}{0.0pt}
\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
GT & 0.2 & 0.4 & 0.3 & 0.4 & 0.4 & 0.4 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 0.3 & 1.0 & 1.3 & 1.0 & 0.4 & 1.0 & 0.6 & 1.6 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.2 & 0.4 & 0.2 & 0.3 & 0.2 & 0.4 & 0.3 & 0.4 & 1.7 & 0.3 & 0.4 \\
\midrule
%mt\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{9DB7D7}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\textbf{ \gls{MINDE}--j ($\sigma=1$)} & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\


%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 3.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{4479BB}} 1.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\textbf{ \gls{MINDE}--j}  & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{4479BB}} 2.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 3.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{4479BB}} 1.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%c\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
\textbf{ \gls{MINDE}--c ($\sigma=1$)} & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

%c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{DAE1EB}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\textbf{ \gls{MINDE}--c} & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
\midrule
MINE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{D53D69}} -1.6 & {\cellcolor[HTML]{D53D69}} -0.4 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{DA5C81}} -0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{D53D69}} -1059.0 & {\cellcolor[HTML]{D53D69}} -4.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
KSG & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{E49AAF}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
LNN & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{628DC4}} 0.9 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.4 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{9DB7D7}} 0.6 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 6.8 & {\cellcolor[HTML]{4479BB}} 33.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.4 & {\cellcolor[HTML]{4479BB}} 7.2 & {\cellcolor[HTML]{DA5C81}} -0.3 & {\cellcolor[HTML]{D53D69}} -0.7 & {\cellcolor[HTML]{9DB7D7}} 0.5 & {\cellcolor[HTML]{4479BB}} 1.1 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 5.5 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
CCA & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{BCCCE1}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=0.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=0.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Mean MI estimates over 10 seeds using N = 10000 samples compared each against the ground-truth. Color indicates relative
negative bias (red) and positive bias (blue). Our method and all neural estimators were trained with 10k training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}

\end{table}


==> tables/10k_sigma_ablations.tex <==
\renewcommand{\tabcolsep}{0.0pt}

\begin{table}
\tiny
\caption{$\sigma$ ablations study with 10k training size. }
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule

gt & 0.2 & 0.4 & 0.3 & 0.4 & 0.4 & 0.4 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 0.3 & 1.0 & 1.3 & 1.0 & 0.4 & 1.0 & 0.6 & 1.6 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.2 & 0.4 & 0.2 & 0.3 & 0.2 & 0.4 & 0.3 & 0.4 & 1.7 & 0.3 & 0.4 \\
mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 3.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{4479BB}} 1.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{4479BB}} 2.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 3.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{4479BB}} 1.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{DAE1EB}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde0.5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E49AAF}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{BCCCE1}} 0.4 & {\cellcolor[HTML]{7FA2CE}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{9DB7D7}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde1.5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{DAE1EB}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{9DB7D7}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{BCCCE1}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{9EB8D8}} 1.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{9DB7D7}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{7FA2CE}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 2.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{7FA2CE}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 2.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{BCCCE1}} 0.4 & {\cellcolor[HTML]{9DB7D7}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{E9BAC8}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde10 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 3.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{7FA2CE}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp0.5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E49AAF}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp1.5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{BCCCE1}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{BCCCE1}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{9EB8D8}} 1.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp3 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{7FA2CE}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 2.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{628DC4}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 2.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp10 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 3.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde0.5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{DAE1EB}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde1.5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} -0.0 & {\cellcolor[HTML]{DF7B98}} -0.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} -0.0 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{EED9DF}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} -0.0 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde10 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{EED9DF}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp0.5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{DAE1EB}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp1.5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{EED9DF}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp10 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{EED9DF}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
MINE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{D53D69}} -1.6 & {\cellcolor[HTML]{D53D69}} -0.4 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{DA5C81}} -0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{D53D69}} -1059.0 & {\cellcolor[HTML]{D53D69}} -4.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
KSG & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{E49AAF}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
LNN & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{628DC4}} 0.9 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.4 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{9DB7D7}} 0.6 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 6.8 & {\cellcolor[HTML]{4479BB}} 33.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.4 & {\cellcolor[HTML]{4479BB}} 7.2 & {\cellcolor[HTML]{DA5C81}} -0.3 & {\cellcolor[HTML]{D53D69}} -0.7 & {\cellcolor[HTML]{9DB7D7}} 0.5 & {\cellcolor[HTML]{4479BB}} 1.1 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 5.5 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
CCA & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{BCCCE1}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=0.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=0.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\

\bottomrule
\end{tabular}
\end{table}


==> tables/stds_tables/10k_std.tex <==
\renewcommand{\tabcolsep}{.0pt}
\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule


%gt & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 \\
%mt\_minde & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{BFCEE2}} .16 & {\cellcolor[HTML]{B3C6DF}} .19 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
mt\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{A8BEDB}} .22 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 \\
%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
%c\_minde & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{7299CA}} .37 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{93B0D4}} .28 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 \\
c\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{6B94C7}} .39 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 \\
%c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{A8BEDB}} .22 & {\cellcolor[HTML]{7CA0CD}} .34 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 \\\midrule
MINE & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 \\
D-V & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{4479BB}} .81 & {\cellcolor[HTML]{4479BB}} 1.91 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{4479BB}} 1.76 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 \\
KSG & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 \\
LNN & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{81A3CE}} .33 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{4479BB}} .56 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 \\
CCA & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{608CC4}} .42 & {\cellcolor[HTML]{4479BB}} 2.04 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{799ECC}} .35 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{85A6D0}} .32 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 \\


 \\dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Standard deviation over 5 seeds using N = 1000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 10k training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}
\label{std_10k}
\end{table}



==> tables/stds_tables/1k_std.tex <==
\renewcommand{\tabcolsep}{.0pt}
\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
%gt & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 \\
%mt\_minde & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{4479BB}} .50 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{A1BAD9}} .24 & {\cellcolor[HTML]{4479BB}} .82 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{4479BB}} 1.54 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{85A6D0}} .32 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{9AB4D6}} .26 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{A8BEDB}} .22 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{AFC4DD}} .20 & {\cellcolor[HTML]{759BCB}} .36 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{648FC5}} .41 & {\cellcolor[HTML]{8FADD3}} .29 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 \\
mt\_minde\_imp & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{4D7FBE}} .47 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{A5BCDA}} .23 & {\cellcolor[HTML]{4479BB}} .63 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{4479BB}} 1.88 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{85A6D0}} .32 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{96B2D5}} .27 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{A8BEDB}} .22 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{6E96C8}} .38 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{6791C6}} .40 & {\cellcolor[HTML]{9AB4D6}} .26 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 \\
%mt\_minde\_s & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{BFCEE2}} .16 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{5987C1}} .44 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{4479BB}} .65 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{8CABD2}} .30 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{AFC4DD}} .20 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{A1BAD9}} .24 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{5B89C2}} .43 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{4479BB}} .54 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{9AB4D6}} .26 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{BBCCE1}} .17 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{BFCEE2}} .16 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 \\
%c\_minde & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{AFC4DD}} .20 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{4479BB}} .89 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{A5BCDA}} .23 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{BFCEE2}} .16 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{AFC4DD}} .20 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{87A8D0}} .31 & {\cellcolor[HTML]{B6C8DF}} .18 & {\cellcolor[HTML]{477BBB}} .49 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{93B0D4}} .28 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 \\
c\_minde\_imp & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{ACC2DC}} .21 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{4479BB}} .81 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{A5BCDA}} .23 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{BBCCE1}} .17 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{AFC4DD}} .20 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{ACC2DC}} .21 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 \\
%c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{7CA0CD}} .34 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{B6C8DF}} .18 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{B6C8DF}} .18 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{DBE2EB}} .08 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{7299CA}} .37 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{AFC4DD}} .20 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{B6C8DF}} .18 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 \\
\midrule
MINE & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{4479BB}} 1.78 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 \\
InfoNCE & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{759BCB}} .36 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{85A6D0}} .32 & {\cellcolor[HTML]{759BCB}} .36 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{4479BB}} 1.01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{4479BB}} .61 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
D-V & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{4479BB}} .58 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{648FC5}} .41 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{A5BCDA}} .23 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{87A8D0}} .31 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{648FC5}} .41 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{7299CA}} .37 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{4479BB}} 1.37 & {\cellcolor[HTML]{4479BB}} 13.13 & {\cellcolor[HTML]{4479BB}} 1.56 & {\cellcolor[HTML]{4479BB}} 2.43 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{4479BB}} 3.07 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
NWJ & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{4479BB}} .64 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{4D7FBE}} .47 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{9AB4D6}} .26 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{4479BB}} .68 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{4479BB}} .72 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{4479BB}} NaN & {\cellcolor[HTML]{4479BB}} NaN & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{4479BB}} NaN & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{4479BB}} NaN & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
KSG & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 \\
LNN & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{B3C6DF}} .19 & {\cellcolor[HTML]{7299CA}} .37 & {\cellcolor[HTML]{4B7DBD}} .48 & {\cellcolor[HTML]{6E96C8}} .38 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 \\
CCA & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{96B2D5}} .27 & {\cellcolor[HTML]{608CC4}} .42 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{AFC4DD}} .20 & {\cellcolor[HTML]{ACC2DC}} .21 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 \\

dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Standard deviation over 5 seeds using N = 1000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 1000 training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}

\end{table}



==> tables/stds_tables/50k_std.tex <==
\renewcommand{\tabcolsep}{.0pt}
\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
%gt & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 \\
%mt\_minde & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{BBCCE1}} .17 & {\cellcolor[HTML]{608CC4}} .42 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 \\
mt\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{648FC5}} .41 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{B3C6DF}} .19 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{BFCEE2}} .16 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
%c\_minde & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{9DB7D7}} .25 & {\cellcolor[HTML]{8CABD2}} .30 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 \\
c\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{B6C8DF}} .18 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 \\
%c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{4D7FBE}} .47 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
\midrule
MINE & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{BFCEE2}} .16 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{C1D0E3}} .15 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 \\
D-V & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{4479BB}} 4.99 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{4479BB}} 9.82 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 \\
KSG & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 \\
LNN & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{BBCCE1}} .17 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{4479BB}} .52 & {\cellcolor[HTML]{BBCCE1}} .17 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 \\
CCA & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{648FC5}} .41 & {\cellcolor[HTML]{4479BB}} 1.27 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\

dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Standard deviation over 5 seeds using N = 10000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 50k training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}
\label{std_50k}
\end{table}



==> tables/stds_tables/5k_std.tex <==
\renewcommand{\tabcolsep}{.0pt}
\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule

%gt & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 & .00 \\
%mt\_minde & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{AFC4DD}} .20 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{96B2D5}} .27 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{BFCEE2}} .16 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 \\
mt\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{ACC2DC}} .21 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{8FADD3}} .29 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 \\
%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{B3C6DF}} .19 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{B3C6DF}} .19 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
%c\_minde & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{9AB4D6}} .26 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{B6C8DF}} .18 & {\cellcolor[HTML]{8FADD3}} .29 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 \\
c\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{96B2D5}} .27 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
%c\_minde\_s & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 \\
\midrule
MINE & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F0F1F2}} .02 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{C6D3E5}} .14 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{E9ECF0}} .04 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
D-V & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{4479BB}} .52 & {\cellcolor[HTML]{4479BB}} 9.73 & {\cellcolor[HTML]{CDD8E7}} .12 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{4479BB}} .91 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{4479BB}} .52 & {\cellcolor[HTML]{4479BB}} .52 & {\cellcolor[HTML]{4479BB}} 89.17 & {\cellcolor[HTML]{D4DDE9}} .10 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{EDEFF1}} .03 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
KSG & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
LNN & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{DBE2EB}} .08 & {\cellcolor[HTML]{C9D5E6}} .13 & {\cellcolor[HTML]{D7DFEA}} .09 & {\cellcolor[HTML]{D0DAE8}} .11 & {\cellcolor[HTML]{E6EAEF}} .05 & {\cellcolor[HTML]{7CA0CD}} .34 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 \\
CCA & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F0F1F2}} .02 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{F2F2F2}} .01 & {\cellcolor[HTML]{4479BB}} .68 & {\cellcolor[HTML]{4479BB}} 1.66 & {\cellcolor[HTML]{E2E7EE}} .06 & {\cellcolor[HTML]{DFE5ED}} .07 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{A5BCDA}} .23 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 & {\cellcolor[HTML]{F2F2F2}} .00 \\



 dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Standard deviation over 5 seeds using N = 5000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 5000 training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}
\label{std_5k}
\end{table}



==> tables/trainsets/results_10k.tex <==
\renewcommand{\tabcolsep}{0.0pt}

\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
gt & 0.2 & 0.4 & 0.3 & 0.4 & 0.4 & 0.4 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 0.3 & 1.0 & 1.3 & 1.0 & 0.4 & 1.0 & 0.6 & 1.6 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.2 & 0.4 & 0.2 & 0.3 & 0.2 & 0.4 & 0.3 & 0.4 & 1.7 & 0.3 & 0.4 \\
\midrule
%mt\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{DAE1EB}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{7FA2CE}} 2.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{7FA2CE}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{DAE1EB}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{7FA2CE}} 2.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{7FA2CE}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{BCCCE1}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{7FA2CE}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{7FA2CE}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{7FA2CE}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{BCCCE1}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{7FA2CE}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{7FA2CE}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%c\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{EED9DF}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{EED9DF}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
\midrule
MINE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{D53D69}} -0.4 & {\cellcolor[HTML]{D53D69}} -0.9 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{D53D69}} -0.8 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
KSG & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{E49AAF}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
LNN & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{628DC4}} 0.9 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.4 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{9DB7D7}} 0.6 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 6.8 & {\cellcolor[HTML]{4479BB}} 33.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.4 & {\cellcolor[HTML]{4479BB}} 7.2 & {\cellcolor[HTML]{DA5C81}} -0.3 & {\cellcolor[HTML]{D53D69}} -0.7 & {\cellcolor[HTML]{9DB7D7}} 0.5 & {\cellcolor[HTML]{4479BB}} 1.0 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 5.5 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
CCA & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{BCCCE1}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{BCCCE1}} 0.4 & {\cellcolor[HTML]{4479BB}} 2.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Mean estimate over 5 seeds using N = 10000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 10k training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}

\end{table}



==> tables/trainsets/results_10k_2.tex <==
\renewcommand{\tabcolsep}{0.0pt}
\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule

gt & 0.22 & 0.43 & 0.29 & 0.45 & 0.41 & 0.41 & 0.41 & 1.02 & 1.02 & 1.02 & 1.02 & 0.29 & 1.02 & 1.29 & 1.02 & 0.41 & 1.02 & 0.59 & 1.62 & 0.41 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 0.22 & 0.43 & 0.19 & 0.29 & 0.18 & 0.45 & 0.30 & 0.41 & 1.71 & 0.33 & 0.41 \\
\midrule
%mt\_minde & {\cellcolor[HTML]{F2EFEF}} 0.19 & {\cellcolor[HTML]{EED6DD}} 0.32 & {\cellcolor[HTML]{F0E3E7}} 0.22 & {\cellcolor[HTML]{F1E9EB}} 0.40 & {\cellcolor[HTML]{F0E3E7}} 0.34 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{D7DFEA}} 1.13 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{D7DFEA}} 1.13 & {\cellcolor[HTML]{CED9E7}} 1.43 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2ECED}} 0.55 & {\cellcolor[HTML]{7FA2CE}} 2.02 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{B2C5DE}} 1.25 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{E6A7B9}} 0.76 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{B9CBE1}} 1.23 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{D1DBE8}} 0.35 & {\cellcolor[HTML]{7CA0CD}} 0.84 & {\cellcolor[HTML]{F2EFEF}} 0.16 & {\cellcolor[HTML]{EAC0CC}} 0.11 & {\cellcolor[HTML]{F2F2F2}} 0.16 & {\cellcolor[HTML]{F1E6E9}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{E6EAEF}} 0.47 & {\cellcolor[HTML]{EFDCE1}} 1.62 & {\cellcolor[HTML]{F1E9EB}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.39 \\
mt\_minde\_imp & {\cellcolor[HTML]{F2EFEF}} 0.19 & {\cellcolor[HTML]{EED9DF}} 0.33 & {\cellcolor[HTML]{F0E3E7}} 0.22 & {\cellcolor[HTML]{F1E9EB}} 0.40 & {\cellcolor[HTML]{F0E3E7}} 0.34 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{D7DFEA}} 1.13 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{D7DFEA}} 1.13 & {\cellcolor[HTML]{D4DDE9}} 1.41 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2EFEF}} 0.56 & {\cellcolor[HTML]{89A9D1}} 1.99 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{B2C5DE}} 1.25 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{E6A7B9}} 0.76 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{B9CBE1}} 1.23 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{E9ECF0}} 0.27 & {\cellcolor[HTML]{D7DFEA}} 0.54 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{EABDCA}} 0.10 & {\cellcolor[HTML]{F2F2F2}} 0.16 & {\cellcolor[HTML]{EFDFE3}} 0.37 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{E6EAEF}} 0.47 & {\cellcolor[HTML]{EFDCE1}} 1.62 & {\cellcolor[HTML]{F1E9EB}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.39 \\
%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{F1E9EB}} 0.38 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{F2F2F2}} 0.45 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{769CCB}} 1.45 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{E9ECF0}} 1.07 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{94B1D5}} 1.35 & {\cellcolor[HTML]{BFCEE2}} 1.48 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 0.61 & {\cellcolor[HTML]{4479BB}} 2.45 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{82A4CF}} 1.41 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{AFC4DD}} 1.26 & {\cellcolor[HTML]{E9BAC8}} 0.82 & {\cellcolor[HTML]{ECCAD4}} 0.87 & {\cellcolor[HTML]{82A4CF}} 1.41 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{EFDFE3}} 0.14 & {\cellcolor[HTML]{EAC0CC}} 0.25 & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{EFF0F2}} 0.32 & {\cellcolor[HTML]{EFF0F2}} 0.21 & {\cellcolor[HTML]{DCE3EC}} 0.54 & {\cellcolor[HTML]{E4E8EE}} 0.37 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 1.70 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{F2ECED}} 0.39 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{F2F2F2}} 0.45 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{799ECC}} 1.44 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{ECEEF1}} 1.06 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{94B1D5}} 1.35 & {\cellcolor[HTML]{BCCCE1}} 1.49 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{EFF0F2}} 0.62 & {\cellcolor[HTML]{4479BB}} 2.46 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{82A4CF}} 1.41 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{B6C8DF}} 1.24 & {\cellcolor[HTML]{E9BAC8}} 0.82 & {\cellcolor[HTML]{ECCAD4}} 0.87 & {\cellcolor[HTML]{82A4CF}} 1.41 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{EED9DF}} 0.12 & {\cellcolor[HTML]{E9B7C6}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{EFF0F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.20 & {\cellcolor[HTML]{DAE1EB}} 0.55 & {\cellcolor[HTML]{E9ECF0}} 0.35 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2EFEF}} 1.68 & {\cellcolor[HTML]{F2EFEF}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
%c\_minde & {\cellcolor[HTML]{F2EFEF}} 0.19 & {\cellcolor[HTML]{F1E9EB}} 0.38 & {\cellcolor[HTML]{F2ECED}} 0.25 & {\cellcolor[HTML]{F2ECED}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{EFF0F2}} 1.05 & {\cellcolor[HTML]{F0E3E7}} 1.22 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.60 & {\cellcolor[HTML]{EDD0D8}} 1.49 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{F2F2F2}} 0.20 & {\cellcolor[HTML]{E6A7B9}} 0.17 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F1E6E9}} 0.23 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F1E6E9}} 0.39 & {\cellcolor[HTML]{F2EFEF}} 0.27 & {\cellcolor[HTML]{EABDCA}} 0.22 & {\cellcolor[HTML]{F1E9EB}} 1.66 & {\cellcolor[HTML]{F2ECED}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
c\_minde\_imp & {\cellcolor[HTML]{F2EFEF}} 0.19 & {\cellcolor[HTML]{F2ECED}} 0.39 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{F2ECED}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{EFDCE1}} 1.20 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.61 & {\cellcolor[HTML]{EED6DD}} 1.51 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EED3DB}} 0.10 & {\cellcolor[HTML]{E6A7B9}} 0.17 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F1E6E9}} 0.23 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F1E6E9}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{EBC6D1}} 0.25 & {\cellcolor[HTML]{EFDCE1}} 1.62 & {\cellcolor[HTML]{F2ECED}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
%c\_minde\_s & {\cellcolor[HTML]{F2EFEF}} 0.19 & {\cellcolor[HTML]{F1E9EB}} 0.38 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{F2EFEF}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{EFF0F2}} 1.05 & {\cellcolor[HTML]{F0E3E7}} 1.22 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.57 & {\cellcolor[HTML]{F2F2F2}} 1.61 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{EFF0F2}} 1.05 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{E7ADBE}} 0.78 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{F2F2F2}} 0.23 & {\cellcolor[HTML]{EDD0D8}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.18 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F2F2F2}} 0.46 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{F1E9EB}} 0.36 & {\cellcolor[HTML]{F1E9EB}} 1.66 & {\cellcolor[HTML]{F2ECED}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F2EFEF}} 0.19 & {\cellcolor[HTML]{F2ECED}} 0.39 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{F2EFEF}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{EFF0F2}} 1.05 & {\cellcolor[HTML]{F1E6E9}} 1.23 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.58 & {\cellcolor[HTML]{F2F2F2}} 1.60 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{EFF0F2}} 1.05 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{EFF0F2}} 1.05 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{EFDCE1}} 0.13 & {\cellcolor[HTML]{E9B7C6}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.19 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F2F2F2}} 0.45 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F1E6E9}} 0.35 & {\cellcolor[HTML]{EFDCE1}} 1.62 & {\cellcolor[HTML]{F2EFEF}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
\midrule
MINE & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F1E9EB}} 0.38 & {\cellcolor[HTML]{EFDCE1}} 0.20 & {\cellcolor[HTML]{ECCAD4}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{ECCAD4}} 0.87 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{F2ECED}} 1.25 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.58 & {\cellcolor[HTML]{F2F2F2}} 1.60 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E9BAC8}} 0.82 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{E5A1B5}} 0.74 & {\cellcolor[HTML]{E188A2}} 0.66 & {\cellcolor[HTML]{DF7B98}} 0.62 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{EBC6D1}} 0.86 & {\cellcolor[HTML]{E9BAC8}} 0.02 & {\cellcolor[HTML]{DE7795}} 0.02 & {\cellcolor[HTML]{EFDCE1}} 0.10 & {\cellcolor[HTML]{EAC0CC}} 0.11 & {\cellcolor[HTML]{F1E6E9}} 0.12 & {\cellcolor[HTML]{E49AAF}} 0.15 & {\cellcolor[HTML]{EDD0D8}} 0.17 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F1E9EB}} 1.66 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.42 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2EFEF}} 0.40 & {\cellcolor[HTML]{F0E3E7}} 0.22 & {\cellcolor[HTML]{EED9DF}} 0.35 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{E9BAC8}} 0.82 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{F2ECED}} 1.25 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.58 & {\cellcolor[HTML]{F1E6E9}} 1.56 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E7AABB}} 0.77 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{E497AD}} 0.71 & {\cellcolor[HTML]{E6A3B7}} 0.75 & {\cellcolor[HTML]{E290A8}} 0.69 & {\cellcolor[HTML]{E6A7B9}} 0.76 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{EDD0D8}} 0.09 & {\cellcolor[HTML]{EABDCA}} 0.24 & {\cellcolor[HTML]{F2EFEF}} 0.16 & {\cellcolor[HTML]{F1E6E9}} 0.23 & {\cellcolor[HTML]{F2ECED}} 0.14 & {\cellcolor[HTML]{EFDFE3}} 0.37 & {\cellcolor[HTML]{EFDCE1}} 0.21 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 1.69 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.42 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2ECED}} 0.39 & {\cellcolor[HTML]{F1E6E9}} 0.23 & {\cellcolor[HTML]{EED9DF}} 0.35 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{EABDCA}} 0.83 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{F2EFEF}} 1.26 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.58 & {\cellcolor[HTML]{F2ECED}} 1.58 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{E49AAF}} 0.72 & {\cellcolor[HTML]{E5A1B5}} 0.74 & {\cellcolor[HTML]{E28BA4}} 0.67 & {\cellcolor[HTML]{E7ADBE}} 0.78 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{E8B4C3}} 0.00 & {\cellcolor[HTML]{DE7493}} 0.01 & {\cellcolor[HTML]{D53F6C}} -0.40 & {\cellcolor[HTML]{D53D69}} -0.91 & {\cellcolor[HTML]{EDD0D8}} 0.05 & {\cellcolor[HTML]{DF7D9A}} 0.06 & {\cellcolor[HTML]{ECCAD4}} 0.15 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 1.69 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2EFEF}} 0.40 & {\cellcolor[HTML]{EFDFE3}} 0.21 & {\cellcolor[HTML]{EED6DD}} 0.34 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{EBC2CE}} 0.85 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{F2EFEF}} 1.26 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.58 & {\cellcolor[HTML]{F0E3E7}} 1.55 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E8B4C3}} 0.80 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{E49AAF}} 0.72 & {\cellcolor[HTML]{E5A1B5}} 0.74 & {\cellcolor[HTML]{E28BA4}} 0.67 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{E9B7C6}} 0.01 & {\cellcolor[HTML]{DD7191}} 0.00 & {\cellcolor[HTML]{EBC6D1}} 0.03 & {\cellcolor[HTML]{D53D69}} -0.78 & {\cellcolor[HTML]{EED3DB}} 0.06 & {\cellcolor[HTML]{DF7D9A}} 0.06 & {\cellcolor[HTML]{EAC0CC}} 0.12 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2EFEF}} 1.68 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
KSG & {\cellcolor[HTML]{F2F2F2}} 0.23 & {\cellcolor[HTML]{F1E9EB}} 0.38 & {\cellcolor[HTML]{EED6DD}} 0.18 & {\cellcolor[HTML]{E9B7C6}} 0.24 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{D53D69}} 0.17 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{E1849F}} 0.65 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{D53D69}} 0.19 & {\cellcolor[HTML]{E8B4C3}} 1.07 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{E5A1B5}} 0.74 & {\cellcolor[HTML]{F2F2F2}} 0.57 & {\cellcolor[HTML]{E290A8}} 1.29 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{D53D69}} 0.20 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{E497AD}} 0.71 & {\cellcolor[HTML]{D53D69}} 0.17 & {\cellcolor[HTML]{E49AAF}} 0.72 & {\cellcolor[HTML]{DB6487}} 0.55 & {\cellcolor[HTML]{D53D69}} 0.19 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{E290A8}} 0.69 & {\cellcolor[HTML]{F1E9EB}} 0.17 & {\cellcolor[HTML]{E9B7C6}} 0.22 & {\cellcolor[HTML]{EED9DF}} 0.09 & {\cellcolor[HTML]{EBC2CE}} 0.12 & {\cellcolor[HTML]{EED6DD}} 0.07 & {\cellcolor[HTML]{E7AABB}} 0.20 & {\cellcolor[HTML]{ECCAD4}} 0.15 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2EFEF}} 1.68 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
LNN & {\cellcolor[HTML]{EFF0F2}} 0.25 & {\cellcolor[HTML]{6C95C8}} 0.89 & {\cellcolor[HTML]{4479BB}} 2.72 & {\cellcolor[HTML]{4479BB}} 6.66 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 2.68 & {\cellcolor[HTML]{4479BB}} 6.45 & {\cellcolor[HTML]{ACC2DC}} 1.27 & {\cellcolor[HTML]{8CABD2}} 0.65 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 3.10 & {\cellcolor[HTML]{4479BB}} 2.48 & {\cellcolor[HTML]{4479BB}} 7.31 & {\cellcolor[HTML]{4479BB}} 6.77 & {\cellcolor[HTML]{4479BB}} 33.48 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 2.49 & {\cellcolor[HTML]{4479BB}} 7.27 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 3.10 & {\cellcolor[HTML]{4479BB}} 7.31 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 2.38 & {\cellcolor[HTML]{4479BB}} 7.24 & {\cellcolor[HTML]{D85179}} -0.31 & {\cellcolor[HTML]{D53D69}} -0.70 & {\cellcolor[HTML]{9DB7D7}} 0.49 & {\cellcolor[HTML]{4479BB}} 1.01 & {\cellcolor[HTML]{4479BB}} 2.11 & {\cellcolor[HTML]{4479BB}} 2.47 & {\cellcolor[HTML]{4479BB}} 5.49 & {\cellcolor[HTML]{F0E3E7}} 0.34 & {\cellcolor[HTML]{E8AFC0}} 1.48 & {\cellcolor[HTML]{F2ECED}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 0.42 \\
CCA & {\cellcolor[HTML]{E8B4C3}} 0.00 & {\cellcolor[HTML]{DD7191}} 0.00 & {\cellcolor[HTML]{E59EB2}} 0.00 & {\cellcolor[HTML]{DC6A8C}} 0.00 & {\cellcolor[HTML]{F0E3E7}} 0.34 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{EFF0F2}} 1.32 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.59 & {\cellcolor[HTML]{D1DBE8}} 1.75 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{EBC2CE}} 0.85 & {\cellcolor[HTML]{D53D69}} 0.23 & {\cellcolor[HTML]{D53D69}} 0.39 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{EAC0CC}} 0.84 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{BCCCE1}} 0.42 & {\cellcolor[HTML]{4479BB}} 2.15 & {\cellcolor[HTML]{F0E3E7}} 0.12 & {\cellcolor[HTML]{DAE1EB}} 0.39 & {\cellcolor[HTML]{EBC2CE}} 0.01 & {\cellcolor[HTML]{EFF0F2}} 0.48 & {\cellcolor[HTML]{E5A1B5}} 0.02 & {\cellcolor[HTML]{DF7D9A}} 0.02 & {\cellcolor[HTML]{EFDFE3}} 1.63 & {\cellcolor[HTML]{ECCAD4}} 0.18 & {\cellcolor[HTML]{F2EFEF}} 0.38 \\dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Mean estimate over 5 seeds using N = 10000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 10000 training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}

\end{table}


==> tables/trainsets/results_1k.tex <==
\renewcommand{\tabcolsep}{0.0pt}

\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
gt & 0.2 & 0.4 & 0.3 & 0.4 & 0.4 & 0.4 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 0.3 & 1.0 & 1.3 & 1.0 & 0.4 & 1.0 & 0.6 & 1.6 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.2 & 0.4 & 0.2 & 0.3 & 0.2 & 0.4 & 0.3 & 0.4 & 1.7 & 0.3 & 0.4 \\
%mt\_minde & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{4479BB}} 2.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 2.4 & {\cellcolor[HTML]{4479BB}} 2.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 8.5 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{4479BB}} 2.3 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{4479BB}} 2.3 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{4479BB}} 2.3 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{7FA2CE}} 0.8 & {\cellcolor[HTML]{DA5C81}} -0.3 & {\cellcolor[HTML]{D53D69}} -0.4 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{D53D69}} -0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{DA5C81}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 \\ \
\midrule
mt\_minde\_imp & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{4479BB}} 2.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 2.4 & {\cellcolor[HTML]{4479BB}} 2.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 8.6 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{4479BB}} 2.3 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{4479BB}} 2.3 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{4479BB}} 2.3 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{9DB7D7}} 0.7 & {\cellcolor[HTML]{DA5C81}} -0.3 & {\cellcolor[HTML]{D53D69}} -0.3 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{D53D69}} -0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{D53D69}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 \\
%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 5.2 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 5.2 & {\cellcolor[HTML]{4479BB}} 5.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{BCCCE1}} 0.8 & {\cellcolor[HTML]{4479BB}} 14.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 5.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{4479BB}} 5.1 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{4479BB}} 5.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{BCCCE1}} 0.4 & {\cellcolor[HTML]{9DB7D7}} 0.6 & {\cellcolor[HTML]{BCCCE1}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.1 & {\cellcolor[HTML]{9DB7D7}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 5.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 5.3 & {\cellcolor[HTML]{4479BB}} 5.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{BCCCE1}} 0.8 & {\cellcolor[HTML]{4479BB}} 14.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 5.1 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{4479BB}} 5.1 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{4479BB}} 5.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{BCCCE1}} 0.4 & {\cellcolor[HTML]{7FA2CE}} 0.7 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.1 & {\cellcolor[HTML]{9DB7D7}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%c\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 2.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{4479BB}} 2.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 0.7 & {\cellcolor[HTML]{4479BB}} 7.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.6 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{4479BB}} 1.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{628DC4}} 1.5 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{E49AAF}} 1.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{4479BB}} 2.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 0.7 & {\cellcolor[HTML]{4479BB}} 7.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.6 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{4479BB}} 1.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{628DC4}} 1.5 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 1.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%c\_minde\_s & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.7 & {\cellcolor[HTML]{BCCCE1}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{628DC4}} 1.5 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{628DC4}} 1.5 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{7FA2CE}} 1.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 1.5 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{BCCCE1}} 1.5 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{628DC4}} 1.5 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{4479BB}} 1.6 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{628DC4}} 1.5 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{E49AAF}} 1.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\ \midrule
MINE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{E9BAC8}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{D53D69}} 0.1 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{D53D69}} -0.8 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} -3.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} -3.3 & {\cellcolor[HTML]{D53D69}} -0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D53D69}} -4.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} -3.5 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{D53D69}} -3.7 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{D53D69}} -3.5 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{D53D69}} -0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E49BB0}} -0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} -0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} -3.5 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} -3.0 & {\cellcolor[HTML]{DA5C81}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D53D69}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} -3.1 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{D53D69}} -3.3 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{D53D69}} -3.2 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{D53D69}} -9.1 & {\cellcolor[HTML]{D53D69}} -6.5 & {\cellcolor[HTML]{D53D69}} -0.8 & {\cellcolor[HTML]{D53D69}} -1.4 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{D53D69}} -2.8 & {\cellcolor[HTML]{DF7B98}} -0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} -0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} -1.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} -2.2 & {\cellcolor[HTML]{DF7B98}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D53D69}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} -2.1 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{D53D69}} -1.8 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{D53D69}} -2.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{D53D69}} NaN & {\cellcolor[HTML]{D53D69}} -129.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{D53D69}} -60.0 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{D53D69}} -1291.3 & {\cellcolor[HTML]{DF7B98}} -0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
KSG & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} 0.1 & {\cellcolor[HTML]{E49AAF}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{EED9DF}} 0.5 & {\cellcolor[HTML]{DF7B98}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{D53D69}} 0.1 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
LNN & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.1 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 6.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 16.9 & {\cellcolor[HTML]{4479BB}} 2.9 & {\cellcolor[HTML]{4479BB}} 5.8 & {\cellcolor[HTML]{628DC4}} 1.5 & {\cellcolor[HTML]{4479BB}} 1.0 & {\cellcolor[HTML]{4479BB}} 16.9 & {\cellcolor[HTML]{4479BB}} 16.9 & {\cellcolor[HTML]{4479BB}} 3.5 & {\cellcolor[HTML]{4479BB}} 3.0 & {\cellcolor[HTML]{4479BB}} 6.3 & {\cellcolor[HTML]{4479BB}} 6.0 & {\cellcolor[HTML]{4479BB}} 33.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 16.9 & {\cellcolor[HTML]{4479BB}} 3.2 & {\cellcolor[HTML]{4479BB}} 6.3 & {\cellcolor[HTML]{4479BB}} 16.9 & {\cellcolor[HTML]{4479BB}} 3.5 & {\cellcolor[HTML]{4479BB}} 6.3 & {\cellcolor[HTML]{4479BB}} 16.9 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 6.3 & {\cellcolor[HTML]{E9BAC8}} -0.0 & {\cellcolor[HTML]{DF7B98}} -0.0 & {\cellcolor[HTML]{4479BB}} 0.8 & {\cellcolor[HTML]{4479BB}} 1.6 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{4479BB}} 3.4 & {\cellcolor[HTML]{4479BB}} 5.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
CCA & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{9DB7D7}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 3.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{9DB7D7}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\ dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Mean estimate over 5 seeds using N = 1000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 1000 training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}

\end{table}


==> tables/trainsets/results_1k_2.tex <==
\renewcommand{\tabcolsep}{0.0pt}
\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
gt & 0.22 & 0.43 & 0.29 & 0.45 & 0.41 & 0.41 & 0.41 & 1.02 & 1.02 & 1.02 & 1.02 & 0.29 & 1.02 & 1.29 & 1.02 & 0.41 & 1.02 & 0.59 & 1.62 & 0.41 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 0.22 & 0.43 & 0.19 & 0.29 & 0.18 & 0.45 & 0.30 & 0.41 & 1.71 & 0.33 & 0.41 \\
\midrule
%mt\_minde & {\cellcolor[HTML]{EDD0D8}} 0.09 & {\cellcolor[HTML]{EABDCA}} 0.24 & {\cellcolor[HTML]{EED6DD}} 0.18 & {\cellcolor[HTML]{EFDCE1}} 0.36 & {\cellcolor[HTML]{E8B4C3}} 0.19 & {\cellcolor[HTML]{EED9DF}} 0.31 & {\cellcolor[HTML]{ECCAD4}} 0.26 & {\cellcolor[HTML]{4479BB}} 2.43 & {\cellcolor[HTML]{EABDCA}} 0.83 & {\cellcolor[HTML]{ECEEF1}} 1.06 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{4479BB}} 2.40 & {\cellcolor[HTML]{4479BB}} 2.04 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{EFF0F2}} 1.05 & {\cellcolor[HTML]{F2F2F2}} 0.61 & {\cellcolor[HTML]{4479BB}} 8.48 & {\cellcolor[HTML]{EFDCE1}} 0.32 & {\cellcolor[HTML]{4479BB}} 2.32 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{4479BB}} 2.28 & {\cellcolor[HTML]{D74B74}} 0.47 & {\cellcolor[HTML]{E188A2}} 0.66 & {\cellcolor[HTML]{4479BB}} 2.29 & {\cellcolor[HTML]{E6A7B9}} 0.76 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{D4DDE9}} 0.34 & {\cellcolor[HTML]{94B1D5}} 0.76 & {\cellcolor[HTML]{D9587E}} -0.32 & {\cellcolor[HTML]{D53D69}} -0.39 & {\cellcolor[HTML]{EED9DF}} 0.08 & {\cellcolor[HTML]{D53D69}} -0.46 & {\cellcolor[HTML]{F2ECED}} 0.26 & {\cellcolor[HTML]{DCE3EC}} 0.50 & {\cellcolor[HTML]{D84E77}} 1.17 & {\cellcolor[HTML]{ECCAD4}} 0.18 & {\cellcolor[HTML]{ECCAD4}} 0.26 \\
mt\_minde\_imp & {\cellcolor[HTML]{ECCDD6}} 0.08 & {\cellcolor[HTML]{E9BAC8}} 0.23 & {\cellcolor[HTML]{EED6DD}} 0.18 & {\cellcolor[HTML]{EFDCE1}} 0.36 & {\cellcolor[HTML]{E9B7C6}} 0.20 & {\cellcolor[HTML]{EFDCE1}} 0.32 & {\cellcolor[HTML]{ECCDD6}} 0.27 & {\cellcolor[HTML]{4479BB}} 2.41 & {\cellcolor[HTML]{EABDCA}} 0.83 & {\cellcolor[HTML]{E4E8EE}} 1.09 & {\cellcolor[HTML]{ECCAD4}} 0.87 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{4479BB}} 2.36 & {\cellcolor[HTML]{4479BB}} 2.02 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{F2ECED}} 0.37 & {\cellcolor[HTML]{E6EAEF}} 1.08 & {\cellcolor[HTML]{ECEEF1}} 0.63 & {\cellcolor[HTML]{4479BB}} 8.58 & {\cellcolor[HTML]{EFDFE3}} 0.33 & {\cellcolor[HTML]{4479BB}} 2.30 & {\cellcolor[HTML]{E7ADBE}} 0.78 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{4479BB}} 2.27 & {\cellcolor[HTML]{D74B74}} 0.47 & {\cellcolor[HTML]{E28BA4}} 0.67 & {\cellcolor[HTML]{4479BB}} 2.27 & {\cellcolor[HTML]{E6A3B7}} 0.75 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{DAE1EB}} 0.32 & {\cellcolor[HTML]{9AB4D6}} 0.74 & {\cellcolor[HTML]{D9557C}} -0.33 & {\cellcolor[HTML]{D53D69}} -0.33 & {\cellcolor[HTML]{EED9DF}} 0.08 & {\cellcolor[HTML]{D53D69}} -0.44 & {\cellcolor[HTML]{F2EFEF}} 0.27 & {\cellcolor[HTML]{DFE5ED}} 0.49 & {\cellcolor[HTML]{D64570}} 1.14 & {\cellcolor[HTML]{ECCAD4}} 0.18 & {\cellcolor[HTML]{ECCDD6}} 0.27 \\
%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.20 & {\cellcolor[HTML]{F0E3E7}} 0.36 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{DCE3EC}} 0.54 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{4479BB}} 5.22 & {\cellcolor[HTML]{D7DFEA}} 1.13 & {\cellcolor[HTML]{97B3D5}} 1.34 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{4479BB}} 5.18 & {\cellcolor[HTML]{4479BB}} 5.41 & {\cellcolor[HTML]{ECEEF1}} 1.06 & {\cellcolor[HTML]{E4E8EE}} 0.48 & {\cellcolor[HTML]{BCCCE1}} 1.22 & {\cellcolor[HTML]{B9CBE1}} 0.80 & {\cellcolor[HTML]{4479BB}} 14.78 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{4479BB}} 5.10 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{BCCCE1}} 1.22 & {\cellcolor[HTML]{4479BB}} 5.05 & {\cellcolor[HTML]{E5A1B5}} 0.74 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{4479BB}} 5.13 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{BFCEE2}} 1.21 & {\cellcolor[HTML]{EFF0F2}} 0.25 & {\cellcolor[HTML]{F0E3E7}} 0.36 & {\cellcolor[HTML]{AFC4DD}} 0.43 & {\cellcolor[HTML]{8CABD2}} 0.65 & {\cellcolor[HTML]{BFCEE2}} 0.37 & {\cellcolor[HTML]{4479BB}} 1.12 & {\cellcolor[HTML]{8FADD3}} 0.65 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{ECCDD6}} 1.57 & {\cellcolor[HTML]{F1E6E9}} 0.27 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.20 & {\cellcolor[HTML]{F1E9EB}} 0.38 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{E6EAEF}} 0.51 & {\cellcolor[HTML]{EFF0F2}} 0.44 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{EFF0F2}} 0.44 & {\cellcolor[HTML]{4479BB}} 5.30 & {\cellcolor[HTML]{D4DDE9}} 1.14 & {\cellcolor[HTML]{9AB4D6}} 1.33 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{EFF0F2}} 0.32 & {\cellcolor[HTML]{4479BB}} 5.26 & {\cellcolor[HTML]{4479BB}} 5.42 & {\cellcolor[HTML]{ECEEF1}} 1.06 & {\cellcolor[HTML]{E9ECF0}} 0.46 & {\cellcolor[HTML]{B9CBE1}} 1.23 & {\cellcolor[HTML]{B9CBE1}} 0.80 & {\cellcolor[HTML]{4479BB}} 14.95 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{4479BB}} 5.14 & {\cellcolor[HTML]{ECEEF1}} 1.06 & {\cellcolor[HTML]{B6C8DF}} 1.24 & {\cellcolor[HTML]{4479BB}} 5.10 & {\cellcolor[HTML]{E49AAF}} 0.72 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{4479BB}} 5.12 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{BFCEE2}} 1.21 & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{EFDCE1}} 0.34 & {\cellcolor[HTML]{B6C8DF}} 0.41 & {\cellcolor[HTML]{89A9D1}} 0.66 & {\cellcolor[HTML]{C7D4E5}} 0.34 & {\cellcolor[HTML]{4479BB}} 1.08 & {\cellcolor[HTML]{9AB4D6}} 0.61 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F1E6E9}} 1.65 & {\cellcolor[HTML]{F1E6E9}} 0.27 & {\cellcolor[HTML]{F2F2F2}} 0.42 \\
%c\_minde & {\cellcolor[HTML]{F0E3E7}} 0.15 & {\cellcolor[HTML]{EDD0D8}} 0.30 & {\cellcolor[HTML]{EFDCE1}} 0.20 & {\cellcolor[HTML]{EFDCE1}} 0.36 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{4479BB}} 2.17 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{4479BB}} 1.94 & {\cellcolor[HTML]{4479BB}} 2.04 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EFF0F2}} 0.44 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{CED9E7}} 0.73 & {\cellcolor[HTML]{4479BB}} 7.03 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{4C7EBD}} 1.59 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{4479BB}} 1.70 & {\cellcolor[HTML]{DC6A8C}} 0.57 & {\cellcolor[HTML]{DE7493}} 0.60 & {\cellcolor[HTML]{628DC4}} 1.52 & {\cellcolor[HTML]{EAC0CC}} 0.84 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{EBC6D1}} 0.06 & {\cellcolor[HTML]{E49BB0}} 0.13 & {\cellcolor[HTML]{CED9E7}} 0.33 & {\cellcolor[HTML]{F0E3E7}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.19 & {\cellcolor[HTML]{DCE3EC}} 0.54 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{E7ADBE}} 0.17 & {\cellcolor[HTML]{E497AD}} 1.40 & {\cellcolor[HTML]{EED9DF}} 0.23 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
c\_minde\_imp & {\cellcolor[HTML]{EFDFE3}} 0.14 & {\cellcolor[HTML]{ECCDD6}} 0.29 & {\cellcolor[HTML]{EFDCE1}} 0.20 & {\cellcolor[HTML]{EED9DF}} 0.35 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{4479BB}} 2.14 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{4479BB}} 1.91 & {\cellcolor[HTML]{4479BB}} 2.04 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{ECEEF1}} 0.45 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{D1DBE8}} 0.72 & {\cellcolor[HTML]{4479BB}} 7.25 & {\cellcolor[HTML]{F1E9EB}} 0.36 & {\cellcolor[HTML]{5786C1}} 1.55 & {\cellcolor[HTML]{EBC2CE}} 0.85 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{4479BB}} 1.67 & {\cellcolor[HTML]{DC6A8C}} 0.57 & {\cellcolor[HTML]{DD7191}} 0.59 & {\cellcolor[HTML]{648FC5}} 1.51 & {\cellcolor[HTML]{E9BAC8}} 0.82 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{EED9DF}} 0.12 & {\cellcolor[HTML]{E290A8}} 0.10 & {\cellcolor[HTML]{EED9DF}} 0.09 & {\cellcolor[HTML]{F1E6E9}} 0.23 & {\cellcolor[HTML]{F2F2F2}} 0.20 & {\cellcolor[HTML]{F2F2F2}} 0.46 & {\cellcolor[HTML]{F2EFEF}} 0.27 & {\cellcolor[HTML]{E5A1B5}} 0.13 & {\cellcolor[HTML]{E6A3B7}} 1.44 & {\cellcolor[HTML]{EED9DF}} 0.23 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
%c\_minde\_s & {\cellcolor[HTML]{EFDCE1}} 0.13 & {\cellcolor[HTML]{EDD0D8}} 0.30 & {\cellcolor[HTML]{F0E3E7}} 0.22 & {\cellcolor[HTML]{EFDCE1}} 0.36 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{4479BB}} 1.82 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{4479BB}} 1.69 & {\cellcolor[HTML]{B2C5DE}} 1.52 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.60 & {\cellcolor[HTML]{4479BB}} 3.07 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{769CCB}} 1.45 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{6A93C7}} 1.49 & {\cellcolor[HTML]{DB6487}} 0.55 & {\cellcolor[HTML]{DE7795}} 0.61 & {\cellcolor[HTML]{7CA0CD}} 1.43 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{E6EAEF}} 0.28 & {\cellcolor[HTML]{F0E3E7}} 0.36 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F2F2F2}} 0.19 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{F0E3E7}} 0.34 & {\cellcolor[HTML]{EAC0CC}} 1.53 & {\cellcolor[HTML]{EED6DD}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.43 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F0E3E7}} 0.15 & {\cellcolor[HTML]{EED3DB}} 0.31 & {\cellcolor[HTML]{F0E3E7}} 0.22 & {\cellcolor[HTML]{EED9DF}} 0.35 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{4479BB}} 1.92 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{4479BB}} 1.77 & {\cellcolor[HTML]{AAC0DC}} 1.55 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{EFF0F2}} 0.62 & {\cellcolor[HTML]{4479BB}} 3.07 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{5E8BC3}} 1.53 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{5585C0}} 1.56 & {\cellcolor[HTML]{DD6F8F}} 0.58 & {\cellcolor[HTML]{DE7795}} 0.61 & {\cellcolor[HTML]{7198C9}} 1.47 & {\cellcolor[HTML]{EBC6D1}} 0.86 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F2ECED}} 0.18 & {\cellcolor[HTML]{EED9DF}} 0.33 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.20 & {\cellcolor[HTML]{F2F2F2}} 0.45 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F1E6E9}} 0.35 & {\cellcolor[HTML]{E6A3B7}} 1.44 & {\cellcolor[HTML]{EFDCE1}} 0.24 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
\midrule
MINE & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{EED6DD}} 0.32 & {\cellcolor[HTML]{E8AFC0}} 0.06 & {\cellcolor[HTML]{DD6F8F}} 0.01 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{EFF0F2}} 0.44 & {\cellcolor[HTML]{D53D69}} 0.11 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{E9ECF0}} 1.07 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{D53D69}} 0.26 & {\cellcolor[HTML]{EBC2CE}} 1.12 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.59 & {\cellcolor[HTML]{E9BAC8}} 1.42 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{D53D69}} 0.29 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{D53D69}} 0.13 & {\cellcolor[HTML]{D9557C}} 0.50 & {\cellcolor[HTML]{D53D69}} 0.42 & {\cellcolor[HTML]{D53D69}} 0.28 & {\cellcolor[HTML]{ECCAD4}} 0.87 & {\cellcolor[HTML]{EAC0CC}} 0.84 & {\cellcolor[HTML]{EED6DD}} 0.11 & {\cellcolor[HTML]{DE7493}} 0.01 & {\cellcolor[HTML]{D53D69}} -0.79 & {\cellcolor[HTML]{E7AABB}} 0.04 & {\cellcolor[HTML]{EDD0D8}} 0.05 & {\cellcolor[HTML]{DC6A8C}} 0.00 & {\cellcolor[HTML]{E59EB2}} 0.01 & {\cellcolor[HTML]{F2ECED}} 0.37 & {\cellcolor[HTML]{EFDFE3}} 1.63 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.42 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{EED3DB}} 0.31 & {\cellcolor[HTML]{E9B7C6}} 0.08 & {\cellcolor[HTML]{DD6F8F}} 0.01 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{D53D69}} -3.38 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{EBC2CE}} 0.85 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{D53D69}} -3.31 & {\cellcolor[HTML]{D53D69}} -0.66 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F2ECED}} 0.37 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{F2ECED}} 0.55 & {\cellcolor[HTML]{D53D69}} -4.01 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{D53D69}} -3.49 & {\cellcolor[HTML]{EAC0CC}} 0.84 & {\cellcolor[HTML]{E8B4C3}} 0.80 & {\cellcolor[HTML]{D53D69}} -3.70 & {\cellcolor[HTML]{D84E77}} 0.48 & {\cellcolor[HTML]{D53D69}} 0.41 & {\cellcolor[HTML]{D53D69}} -3.47 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{E6A7B9}} 0.76 & {\cellcolor[HTML]{EED6DD}} 0.11 & {\cellcolor[HTML]{D53D69}} -0.19 & {\cellcolor[HTML]{EFDFE3}} 0.11 & {\cellcolor[HTML]{E9B7C6}} 0.08 & {\cellcolor[HTML]{EED3DB}} 0.06 & {\cellcolor[HTML]{DF7B98}} 0.05 & {\cellcolor[HTML]{E497AD}} -0.01 & {\cellcolor[HTML]{F2ECED}} 0.37 & {\cellcolor[HTML]{F2ECED}} 1.67 & {\cellcolor[HTML]{F2EFEF}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{EDD0D8}} 0.30 & {\cellcolor[HTML]{E7ADBE}} 0.05 & {\cellcolor[HTML]{DB6185}} -0.03 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{D53D69}} -3.53 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{EBC2CE}} 0.85 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{D53D69}} -3.02 & {\cellcolor[HTML]{D85179}} 0.76 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F2ECED}} 0.37 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{F2ECED}} 0.55 & {\cellcolor[HTML]{D53D69}} 0.52 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{D53D69}} -3.07 & {\cellcolor[HTML]{EBC2CE}} 0.85 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{D53D69}} -3.28 & {\cellcolor[HTML]{D74872}} 0.46 & {\cellcolor[HTML]{D53D69}} 0.40 & {\cellcolor[HTML]{D53D69}} -3.19 & {\cellcolor[HTML]{E9BAC8}} 0.82 & {\cellcolor[HTML]{E7AABB}} 0.77 & {\cellcolor[HTML]{D53D69}} -9.13 & {\cellcolor[HTML]{D53D69}} -6.52 & {\cellcolor[HTML]{D53D69}} -0.79 & {\cellcolor[HTML]{D53D69}} -1.36 & {\cellcolor[HTML]{ECCAD4}} 0.03 & {\cellcolor[HTML]{D53D69}} -2.77 & {\cellcolor[HTML]{DF7D9A}} -0.09 & {\cellcolor[HTML]{F2ECED}} 0.37 & {\cellcolor[HTML]{F1E9EB}} 1.66 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{EDD0D8}} 0.30 & {\cellcolor[HTML]{E7ADBE}} 0.05 & {\cellcolor[HTML]{DC6789}} -0.01 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{D53D69}} -1.88 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{EBC2CE}} 0.85 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{D53D69}} -2.21 & {\cellcolor[HTML]{DE7795}} 0.88 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F2ECED}} 0.37 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{F2ECED}} 0.55 & {\cellcolor[HTML]{D53D69}} 0.78 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{D53D69}} -2.09 & {\cellcolor[HTML]{EBC2CE}} 0.85 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{D53D69}} -1.78 & {\cellcolor[HTML]{D74872}} 0.46 & {\cellcolor[HTML]{D53D69}} 0.40 & {\cellcolor[HTML]{D53D69}} -1.96 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{E7AABB}} 0.77 & {\cellcolor[HTML]{D53D69}} -8548915035.05 & {\cellcolor[HTML]{D53D69}} -129.91 & {\cellcolor[HTML]{EED6DD}} 0.08 & {\cellcolor[HTML]{D53D69}} -60.00 & {\cellcolor[HTML]{EBC6D1}} 0.02 & {\cellcolor[HTML]{D53D69}} -1291.32 & {\cellcolor[HTML]{E1849F}} -0.07 & {\cellcolor[HTML]{F2ECED}} 0.37 & {\cellcolor[HTML]{F1E9EB}} 1.66 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
KSG & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{EABDCA}} 0.24 & {\cellcolor[HTML]{ECCDD6}} 0.15 & {\cellcolor[HTML]{E9BAC8}} 0.25 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{D53D69}} 0.09 & {\cellcolor[HTML]{E393AB}} 0.70 & {\cellcolor[HTML]{D84E77}} 0.48 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{D53D69}} 0.12 & {\cellcolor[HTML]{E290A8}} 0.96 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{DB6185}} 0.54 & {\cellcolor[HTML]{F0E3E7}} 0.52 & {\cellcolor[HTML]{DC6A8C}} 1.17 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{D53D69}} 0.13 & {\cellcolor[HTML]{E7ADBE}} 0.78 & {\cellcolor[HTML]{DB6185}} 0.54 & {\cellcolor[HTML]{D53D69}} 0.12 & {\cellcolor[HTML]{DA5C81}} 0.52 & {\cellcolor[HTML]{D53D69}} 0.39 & {\cellcolor[HTML]{D53D69}} 0.13 & {\cellcolor[HTML]{E5A1B5}} 0.74 & {\cellcolor[HTML]{D9557C}} 0.50 & {\cellcolor[HTML]{EED3DB}} 0.10 & {\cellcolor[HTML]{E59EB2}} 0.14 & {\cellcolor[HTML]{EED3DB}} 0.07 & {\cellcolor[HTML]{ECCAD4}} 0.14 & {\cellcolor[HTML]{EED9DF}} 0.08 & {\cellcolor[HTML]{E9BAC8}} 0.25 & {\cellcolor[HTML]{EED9DF}} 0.20 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{EED6DD}} 1.60 & {\cellcolor[HTML]{F2ECED}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
LNN & {\cellcolor[HTML]{DFE5ED}} 0.30 & {\cellcolor[HTML]{4479BB}} 1.14 & {\cellcolor[HTML]{4479BB}} 3.10 & {\cellcolor[HTML]{4479BB}} 5.98 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{EFF0F2}} 0.44 & {\cellcolor[HTML]{4479BB}} 16.88 & {\cellcolor[HTML]{4479BB}} 2.92 & {\cellcolor[HTML]{4479BB}} 5.80 & {\cellcolor[HTML]{6C95C8}} 1.48 & {\cellcolor[HTML]{4479BB}} 0.99 & {\cellcolor[HTML]{4479BB}} 16.88 & {\cellcolor[HTML]{4479BB}} 16.88 & {\cellcolor[HTML]{4479BB}} 3.50 & {\cellcolor[HTML]{4479BB}} 2.98 & {\cellcolor[HTML]{4479BB}} 6.31 & {\cellcolor[HTML]{4479BB}} 6.04 & {\cellcolor[HTML]{4479BB}} 33.23 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{4479BB}} 16.88 & {\cellcolor[HTML]{4479BB}} 3.19 & {\cellcolor[HTML]{4479BB}} 6.29 & {\cellcolor[HTML]{4479BB}} 16.88 & {\cellcolor[HTML]{4479BB}} 3.51 & {\cellcolor[HTML]{4479BB}} 6.31 & {\cellcolor[HTML]{4479BB}} 16.88 & {\cellcolor[HTML]{4479BB}} 3.10 & {\cellcolor[HTML]{4479BB}} 6.28 & {\cellcolor[HTML]{E7AABB}} -0.03 & {\cellcolor[HTML]{DB6487}} -0.04 & {\cellcolor[HTML]{4479BB}} 0.84 & {\cellcolor[HTML]{4479BB}} 1.60 & {\cellcolor[HTML]{4479BB}} 2.14 & {\cellcolor[HTML]{4479BB}} 3.43 & {\cellcolor[HTML]{4479BB}} 4.97 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{E28EA6}} 1.37 & {\cellcolor[HTML]{F1E9EB}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.42 \\
CCA & {\cellcolor[HTML]{E8B4C3}} 0.00 & {\cellcolor[HTML]{DE7493}} 0.01 & {\cellcolor[HTML]{E5A1B5}} 0.01 & {\cellcolor[HTML]{DD7191}} 0.02 & {\cellcolor[HTML]{EFDFE3}} 0.33 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{AFC4DD}} 1.26 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{97B3D5}} 1.34 & {\cellcolor[HTML]{97B3D5}} 1.61 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{F2F2F2}} 0.60 & {\cellcolor[HTML]{4479BB}} 2.98 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{A6BDDA}} 1.29 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{CED9E7}} 1.16 & {\cellcolor[HTML]{D53D69}} 0.25 & {\cellcolor[HTML]{D53D69}} 0.41 & {\cellcolor[HTML]{AAC0DC}} 1.28 & {\cellcolor[HTML]{EBC2CE}} 0.85 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{F1E9EB}} 0.17 & {\cellcolor[HTML]{AFC4DD}} 0.67 & {\cellcolor[HTML]{EBC2CE}} 0.02 & {\cellcolor[HTML]{EDD0D8}} 0.16 & {\cellcolor[HTML]{F1E6E9}} 0.12 & {\cellcolor[HTML]{F2ECED}} 0.41 & {\cellcolor[HTML]{F0E3E7}} 0.23 & {\cellcolor[HTML]{DF7D9A}} 0.02 & {\cellcolor[HTML]{EFDCE1}} 1.62 & {\cellcolor[HTML]{ECCAD4}} 0.18 & {\cellcolor[HTML]{F2ECED}} 0.37 \\dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Mean estimate over 5 seeds using N = 1000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 1000 training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}

\end{table}



==> tables/trainsets/results_50k.tex <==

\renewcommand{\tabcolsep}{0.0pt}
\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
gt & 0.2 & 0.4 & 0.3 & 0.4 & 0.4 & 0.4 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 0.3 & 1.0 & 1.3 & 1.0 & 0.4 & 1.0 & 0.6 & 1.6 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.2 & 0.4 & 0.2 & 0.3 & 0.2 & 0.4 & 0.3 & 0.4 & 1.7 & 0.3 & 0.4 \\
\midrule
%mt\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{BCCCE1}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{BCCCE1}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{BCCCE1}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{BCCCE1}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%c\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\ \midrule
MINE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{D53D69}} -2.4 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{D53D69}} -6.0 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
KSG & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{E49AAF}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
LNN & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{628DC4}} 0.9 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 6.4 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{7FA2CE}} 0.7 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 6.8 & {\cellcolor[HTML]{4479BB}} 33.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 3.1 & {\cellcolor[HTML]{4479BB}} 7.3 & {\cellcolor[HTML]{4479BB}} 17.3 & {\cellcolor[HTML]{4479BB}} 2.4 & {\cellcolor[HTML]{4479BB}} 7.2 & {\cellcolor[HTML]{DA5C81}} -0.3 & {\cellcolor[HTML]{D53D69}} -0.6 & {\cellcolor[HTML]{7FA2CE}} 0.6 & {\cellcolor[HTML]{4479BB}} 1.2 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{4479BB}} 3.0 & {\cellcolor[HTML]{4479BB}} 5.4 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
CCA & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{BCCCE1}} 1.8 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{9DB7D7}} 0.5 & {\cellcolor[HTML]{4479BB}} 1.4 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Mean estimate over 5 seeds using N = 10000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 50k training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}

\end{table}



==> tables/trainsets/results_50k_2.tex <==
\renewcommand{\tabcolsep}{0.0pt}
\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}

\toprule
gt & 0.22 & 0.43 & 0.29 & 0.45 & 0.41 & 0.41 & 0.41 & 1.02 & 1.02 & 1.02 & 1.02 & 0.29 & 1.02 & 1.29 & 1.02 & 0.41 & 1.02 & 0.59 & 1.62 & 0.41 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 0.22 & 0.43 & 0.19 & 0.29 & 0.18 & 0.45 & 0.30 & 0.41 & 1.71 & 0.33 & 0.41 \\
\midrule
%mt\_minde & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{F2EFEF}} 0.40 & {\cellcolor[HTML]{F2ECED}} 0.25 & {\cellcolor[HTML]{EFDCE1}} 0.36 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{DFE5ED}} 1.10 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{EED3DB}} 1.17 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.59 & {\cellcolor[HTML]{C1D0E3}} 1.80 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{D4DDE9}} 0.34 & {\cellcolor[HTML]{EAC0CC}} 0.25 & {\cellcolor[HTML]{F1E9EB}} 0.14 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{F2F2F2}} 0.16 & {\cellcolor[HTML]{F2EFEF}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{E4E8EE}} 0.48 & {\cellcolor[HTML]{EED9DF}} 1.61 & {\cellcolor[HTML]{F2EFEF}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
mt\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{F2ECED}} 0.39 & {\cellcolor[HTML]{F2ECED}} 0.25 & {\cellcolor[HTML]{EFDCE1}} 0.36 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{DCE3EC}} 1.11 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{EDD0D8}} 1.16 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.59 & {\cellcolor[HTML]{B6C8DF}} 1.84 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F0E3E7}} 0.15 & {\cellcolor[HTML]{E6A7B9}} 0.17 & {\cellcolor[HTML]{F1E9EB}} 0.14 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.16 & {\cellcolor[HTML]{F2EFEF}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{E4E8EE}} 0.48 & {\cellcolor[HTML]{F0E3E7}} 1.64 & {\cellcolor[HTML]{F2EFEF}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F2ECED}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{C1D0E3}} 1.20 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 1.31 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.60 & {\cellcolor[HTML]{C7D4E5}} 1.78 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{DCE3EC}} 1.11 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{DFE5ED}} 1.10 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F0E3E7}} 0.15 & {\cellcolor[HTML]{EBC6D1}} 0.27 & {\cellcolor[HTML]{F2F2F2}} 0.19 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.18 & {\cellcolor[HTML]{F2F2F2}} 0.46 & {\cellcolor[HTML]{EFF0F2}} 0.33 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 1.69 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F2EFEF}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{C4D2E4}} 1.19 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 1.31 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.60 & {\cellcolor[HTML]{C4D2E4}} 1.79 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{DFE5ED}} 1.10 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{E4E8EE}} 1.09 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{EED9DF}} 0.12 & {\cellcolor[HTML]{E8B4C3}} 0.21 & {\cellcolor[HTML]{F2F2F2}} 0.19 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 0.18 & {\cellcolor[HTML]{F2F2F2}} 0.47 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F1E9EB}} 1.66 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
%c\_minde & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F2ECED}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2ECED}} 1.25 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.60 & {\cellcolor[HTML]{F2F2F2}} 1.64 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{EBC6D1}} 0.06 & {\cellcolor[HTML]{E9B7C6}} 0.22 & {\cellcolor[HTML]{F2EFEF}} 0.16 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.18 & {\cellcolor[HTML]{F2EFEF}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{ECCAD4}} 0.26 & {\cellcolor[HTML]{F1E9EB}} 1.66 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
c\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F1E9EB}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F1E6E9}} 1.23 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.60 & {\cellcolor[HTML]{F2F2F2}} 1.64 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{EED3DB}} 0.10 & {\cellcolor[HTML]{E9BAC8}} 0.23 & {\cellcolor[HTML]{F2EFEF}} 0.16 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.18 & {\cellcolor[HTML]{F1E6E9}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{EFDCE1}} 0.32 & {\cellcolor[HTML]{F1E9EB}} 1.66 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.42 \\
%c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F2ECED}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2EFEF}} 1.26 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.59 & {\cellcolor[HTML]{F2F2F2}} 1.60 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{EED9DF}} 0.12 & {\cellcolor[HTML]{F2F2F2}} 0.44 & {\cellcolor[HTML]{F2F2F2}} 0.18 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.18 & {\cellcolor[HTML]{F2F2F2}} 0.44 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F0E3E7}} 1.64 & {\cellcolor[HTML]{F2EFEF}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F2EFEF}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2EFEF}} 1.26 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.58 & {\cellcolor[HTML]{F2EFEF}} 1.59 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{EED6DD}} 0.11 & {\cellcolor[HTML]{E8AFC0}} 0.20 & {\cellcolor[HTML]{F2F2F2}} 0.18 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F2F2F2}} 0.44 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F0E3E7}} 1.64 & {\cellcolor[HTML]{F2EFEF}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\ \midrule
MINE & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F1E6E9}} 0.37 & {\cellcolor[HTML]{F0E3E7}} 0.22 & {\cellcolor[HTML]{EED9DF}} 0.35 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2EFEF}} 1.26 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.60 & {\cellcolor[HTML]{F2F2F2}} 1.60 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{ECCAD4}} 0.87 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{E188A2}} 0.66 & {\cellcolor[HTML]{E188A2}} 0.66 & {\cellcolor[HTML]{EBC2CE}} 0.85 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EBC6D1}} 0.86 & {\cellcolor[HTML]{EABDCA}} 0.03 & {\cellcolor[HTML]{DE7493}} 0.01 & {\cellcolor[HTML]{F0E3E7}} 0.12 & {\cellcolor[HTML]{ECCAD4}} 0.14 & {\cellcolor[HTML]{F1E6E9}} 0.12 & {\cellcolor[HTML]{E5A1B5}} 0.17 & {\cellcolor[HTML]{EDD0D8}} 0.17 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2EFEF}} 1.68 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{F1E9EB}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 1.27 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.59 & {\cellcolor[HTML]{F2F2F2}} 1.60 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{EAC0CC}} 0.84 & {\cellcolor[HTML]{E8B4C3}} 0.80 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{EED9DF}} 0.12 & {\cellcolor[HTML]{ECCAD4}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.18 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F2EFEF}} 0.15 & {\cellcolor[HTML]{F2ECED}} 0.41 & {\cellcolor[HTML]{F2EFEF}} 0.27 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 1.69 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F1E9EB}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 1.27 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.59 & {\cellcolor[HTML]{F2F2F2}} 1.60 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{E9B7C6}} 0.01 & {\cellcolor[HTML]{DE7493}} 0.01 & {\cellcolor[HTML]{D53D69}} -2.36 & {\cellcolor[HTML]{E6A7B9}} 0.03 & {\cellcolor[HTML]{F0E3E7}} 0.11 & {\cellcolor[HTML]{E188A2}} 0.09 & {\cellcolor[HTML]{EFDFE3}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 1.69 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{F1E9EB}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 1.27 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.59 & {\cellcolor[HTML]{F2EFEF}} 1.59 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{E8B4C3}} 0.80 & {\cellcolor[HTML]{E7ADBE}} 0.78 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{E9B7C6}} 0.01 & {\cellcolor[HTML]{DE7795}} 0.02 & {\cellcolor[HTML]{D53D69}} -5.97 & {\cellcolor[HTML]{E7ADBE}} 0.05 & {\cellcolor[HTML]{F0E3E7}} 0.11 & {\cellcolor[HTML]{DF7B98}} 0.05 & {\cellcolor[HTML]{EBC6D1}} 0.14 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 1.69 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
KSG & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F1E9EB}} 0.38 & {\cellcolor[HTML]{EED9DF}} 0.19 & {\cellcolor[HTML]{E9B7C6}} 0.24 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{D53D69}} 0.16 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{E188A2}} 0.66 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{D53D69}} 0.19 & {\cellcolor[HTML]{E8B4C3}} 1.07 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E5A1B5}} 0.74 & {\cellcolor[HTML]{F2F2F2}} 0.57 & {\cellcolor[HTML]{E28EA6}} 1.28 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{D53D69}} 0.20 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{E49AAF}} 0.72 & {\cellcolor[HTML]{D53D69}} 0.17 & {\cellcolor[HTML]{E497AD}} 0.71 & {\cellcolor[HTML]{DB6487}} 0.55 & {\cellcolor[HTML]{D53D69}} 0.19 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{E290A8}} 0.69 & {\cellcolor[HTML]{F1E6E9}} 0.16 & {\cellcolor[HTML]{E9BAC8}} 0.23 & {\cellcolor[HTML]{EED9DF}} 0.09 & {\cellcolor[HTML]{EBC2CE}} 0.12 & {\cellcolor[HTML]{EED6DD}} 0.07 & {\cellcolor[HTML]{E6A7B9}} 0.19 & {\cellcolor[HTML]{EBC6D1}} 0.14 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2EFEF}} 1.68 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.42 \\
LNN & {\cellcolor[HTML]{F2F2F2}} 0.24 & {\cellcolor[HTML]{6C95C8}} 0.89 & {\cellcolor[HTML]{4479BB}} 2.71 & {\cellcolor[HTML]{4479BB}} 6.66 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 2.67 & {\cellcolor[HTML]{4479BB}} 6.45 & {\cellcolor[HTML]{ACC2DC}} 1.27 & {\cellcolor[HTML]{89A9D1}} 0.66 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 3.10 & {\cellcolor[HTML]{4479BB}} 2.48 & {\cellcolor[HTML]{4479BB}} 7.32 & {\cellcolor[HTML]{4479BB}} 6.75 & {\cellcolor[HTML]{4479BB}} 33.48 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 2.49 & {\cellcolor[HTML]{4479BB}} 7.28 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 3.10 & {\cellcolor[HTML]{4479BB}} 7.32 & {\cellcolor[HTML]{4479BB}} 17.34 & {\cellcolor[HTML]{4479BB}} 2.38 & {\cellcolor[HTML]{4479BB}} 7.25 & {\cellcolor[HTML]{DB6185}} -0.26 & {\cellcolor[HTML]{D53D69}} -0.63 & {\cellcolor[HTML]{8CABD2}} 0.55 & {\cellcolor[HTML]{4479BB}} 1.18 & {\cellcolor[HTML]{4479BB}} 2.11 & {\cellcolor[HTML]{4479BB}} 2.96 & {\cellcolor[HTML]{4479BB}} 5.41 & {\cellcolor[HTML]{F0E3E7}} 0.34 & {\cellcolor[HTML]{E8AFC0}} 1.48 & {\cellcolor[HTML]{F2ECED}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 0.42 \\
CCA & {\cellcolor[HTML]{E8B4C3}} 0.00 & {\cellcolor[HTML]{DD7191}} 0.00 & {\cellcolor[HTML]{E59EB2}} 0.00 & {\cellcolor[HTML]{DC6A8C}} 0.00 & {\cellcolor[HTML]{F0E3E7}} 0.34 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{ECEEF1}} 1.06 & {\cellcolor[HTML]{EFF0F2}} 1.32 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.60 & {\cellcolor[HTML]{D1DBE8}} 1.75 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{EBC6D1}} 0.86 & {\cellcolor[HTML]{D53D69}} 0.24 & {\cellcolor[HTML]{D53D69}} 0.39 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{EAC0CC}} 0.84 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{A4BCDA}} 0.50 & {\cellcolor[HTML]{4479BB}} 1.36 & {\cellcolor[HTML]{ECCDD6}} 0.05 & {\cellcolor[HTML]{EBC6D1}} 0.13 & {\cellcolor[HTML]{EBC2CE}} 0.01 & {\cellcolor[HTML]{E8B4C3}} 0.23 & {\cellcolor[HTML]{E6A3B7}} 0.03 & {\cellcolor[HTML]{DF7D9A}} 0.02 & {\cellcolor[HTML]{EFDFE3}} 1.63 & {\cellcolor[HTML]{ECCAD4}} 0.18 & {\cellcolor[HTML]{F2EFEF}} 0.38 \\dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Mean estimate over 5 seeds using N = 10000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 50k training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}

\end{table}



==> tables/trainsets/results_5k.tex <==
\renewcommand{\tabcolsep}{0.0pt}

\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
gt & 0.2 & 0.4 & 0.3 & 0.4 & 0.4 & 0.4 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 0.3 & 1.0 & 1.3 & 1.0 & 0.4 & 1.0 & 0.6 & 1.6 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.2 & 0.4 & 0.2 & 0.3 & 0.2 & 0.4 & 0.3 & 0.4 & 1.7 & 0.3 & 0.4 \\
%mt\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{628DC4}} 1.5 & {\cellcolor[HTML]{BCCCE1}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.5 & {\cellcolor[HTML]{4479BB}} 3.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{7FA2CE}} 1.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{7FA2CE}} 1.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49BB0}} -0.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\ 
\midrule
mt\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{628DC4}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{628DC4}} 1.5 & {\cellcolor[HTML]{BCCCE1}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.5 & {\cellcolor[HTML]{4479BB}} 3.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{7FA2CE}} 1.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{7FA2CE}} 1.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49BB0}} -0.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 2.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{4479BB}} 2.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 4.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{4479BB}} 2.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{BCCCE1}} 0.6 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 2.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{4479BB}} 2.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{4479BB}} 4.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{4479BB}} 1.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{4479BB}} 2.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{BCCCE1}} 0.6 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%c\_minde & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{DAE1EB}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{DAE1EB}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
%c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{DAE1EB}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{DAE1EB}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{BCCCE1}} 1.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
\midrule
MINE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E49AAF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{E9BAC8}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{EED9DF}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DF7B98}} -0.2 & {\cellcolor[HTML]{D53D69}} -4.8 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{D53D69}} -0.6 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{EED9DF}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DA5C81}} -0.3 & {\cellcolor[HTML]{D53D69}} -0.2 & {\cellcolor[HTML]{D53D69}} -44.5 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
KSG & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E49AAF}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{DF7B98}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
LNN & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{4479BB}} 1.0 & {\cellcolor[HTML]{4479BB}} 2.8 & {\cellcolor[HTML]{4479BB}} 6.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.2 & {\cellcolor[HTML]{4479BB}} 2.8 & {\cellcolor[HTML]{4479BB}} 6.3 & {\cellcolor[HTML]{9DB7D7}} 1.3 & {\cellcolor[HTML]{7FA2CE}} 0.7 & {\cellcolor[HTML]{4479BB}} 17.2 & {\cellcolor[HTML]{4479BB}} 17.2 & {\cellcolor[HTML]{4479BB}} 3.2 & {\cellcolor[HTML]{4479BB}} 2.6 & {\cellcolor[HTML]{4479BB}} 7.0 & {\cellcolor[HTML]{4479BB}} 6.6 & {\cellcolor[HTML]{4479BB}} 33.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{4479BB}} 17.2 & {\cellcolor[HTML]{4479BB}} 2.7 & {\cellcolor[HTML]{4479BB}} 7.0 & {\cellcolor[HTML]{4479BB}} 17.2 & {\cellcolor[HTML]{4479BB}} 3.3 & {\cellcolor[HTML]{4479BB}} 7.0 & {\cellcolor[HTML]{4479BB}} 17.2 & {\cellcolor[HTML]{4479BB}} 2.6 & {\cellcolor[HTML]{4479BB}} 7.0 & {\cellcolor[HTML]{DF7B98}} -0.2 & {\cellcolor[HTML]{D53D69}} -0.6 & {\cellcolor[HTML]{7FA2CE}} 0.6 & {\cellcolor[HTML]{4479BB}} 1.4 & {\cellcolor[HTML]{4479BB}} 2.2 & {\cellcolor[HTML]{4479BB}} 3.0 & {\cellcolor[HTML]{4479BB}} 5.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
CCA & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{DAE1EB}} 1.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{9EB8D8}} 1.9 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{D53D69}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{9DB7D7}} 0.5 & {\cellcolor[HTML]{4479BB}} 2.2 & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49BB0}} 0.0 & {\cellcolor[HTML]{DF7B98}} 0.0 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Mean estimate over 5 seeds using N = 5000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 5000 training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}

\end{table}



==> tables/trainsets/results_5k_2.tex <==
\renewcommand{\tabcolsep}{0.0pt}

\begin{table}
\tiny
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
gt & 0.22 & 0.43 & 0.29 & 0.45 & 0.41 & 0.41 & 0.41 & 1.02 & 1.02 & 1.02 & 1.02 & 0.29 & 1.02 & 1.29 & 1.02 & 0.41 & 1.02 & 0.59 & 1.62 & 0.41 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 1.02 & 0.22 & 0.43 & 0.19 & 0.29 & 0.18 & 0.45 & 0.30 & 0.41 & 1.71 & 0.33 & 0.41 \\
\midrule
%mt\_minde & {\cellcolor[HTML]{F2EFEF}} 0.19 & {\cellcolor[HTML]{EFDCE1}} 0.34 & {\cellcolor[HTML]{F0E3E7}} 0.22 & {\cellcolor[HTML]{F2EFEF}} 0.42 & {\cellcolor[HTML]{EFDFE3}} 0.33 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{5786C1}} 1.55 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{6C95C8}} 1.48 & {\cellcolor[HTML]{BCCCE1}} 1.49 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F1E9EB}} 0.54 & {\cellcolor[HTML]{4479BB}} 2.97 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{7CA0CD}} 1.43 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{A6BDDA}} 1.29 & {\cellcolor[HTML]{E497AD}} 0.71 & {\cellcolor[HTML]{E5A1B5}} 0.74 & {\cellcolor[HTML]{7CA0CD}} 1.43 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{E9ECF0}} 0.27 & {\cellcolor[HTML]{E6EAEF}} 0.49 & {\cellcolor[HTML]{EED3DB}} 0.07 & {\cellcolor[HTML]{E290A8}} -0.04 & {\cellcolor[HTML]{F2EFEF}} 0.15 & {\cellcolor[HTML]{EDD0D8}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{DCE3EC}} 0.50 & {\cellcolor[HTML]{EED3DB}} 1.59 & {\cellcolor[HTML]{F1E9EB}} 0.28 & {\cellcolor[HTML]{F2EFEF}} 0.38 \\
mt\_minde\_imp & {\cellcolor[HTML]{F2ECED}} 0.18 & {\cellcolor[HTML]{EFDCE1}} 0.34 & {\cellcolor[HTML]{F0E3E7}} 0.22 & {\cellcolor[HTML]{F2ECED}} 0.41 & {\cellcolor[HTML]{F0E3E7}} 0.34 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{5B89C2}} 1.54 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{749ACA}} 1.46 & {\cellcolor[HTML]{C4D2E4}} 1.46 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F1E9EB}} 0.54 & {\cellcolor[HTML]{4479BB}} 2.98 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{82A4CF}} 1.41 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{ACC2DC}} 1.27 & {\cellcolor[HTML]{E393AB}} 0.70 & {\cellcolor[HTML]{E5A1B5}} 0.74 & {\cellcolor[HTML]{82A4CF}} 1.41 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F2F2F2}} 0.23 & {\cellcolor[HTML]{E6EAEF}} 0.49 & {\cellcolor[HTML]{EED3DB}} 0.07 & {\cellcolor[HTML]{E393AB}} -0.03 & {\cellcolor[HTML]{F2ECED}} 0.14 & {\cellcolor[HTML]{EED3DB}} 0.33 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{DFE5ED}} 0.49 & {\cellcolor[HTML]{EDD0D8}} 1.58 & {\cellcolor[HTML]{F1E9EB}} 0.28 & {\cellcolor[HTML]{F2EFEF}} 0.38 \\
%mt\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2ECED}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F2F2F2}} 0.47 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{4479BB}} 2.23 & {\cellcolor[HTML]{EFF0F2}} 1.05 & {\cellcolor[HTML]{DFE5ED}} 1.10 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{4479BB}} 2.12 & {\cellcolor[HTML]{4479BB}} 2.19 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{ECEEF1}} 1.06 & {\cellcolor[HTML]{EFF0F2}} 0.62 & {\cellcolor[HTML]{4479BB}} 4.43 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{4479BB}} 2.08 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{ECEEF1}} 1.06 & {\cellcolor[HTML]{4479BB}} 1.95 & {\cellcolor[HTML]{E8B4C3}} 0.80 & {\cellcolor[HTML]{EAC0CC}} 0.84 & {\cellcolor[HTML]{4479BB}} 2.12 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{ECEEF1}} 1.06 & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{F0E3E7}} 0.36 & {\cellcolor[HTML]{EFF0F2}} 0.22 & {\cellcolor[HTML]{E4E8EE}} 0.36 & {\cellcolor[HTML]{F2F2F2}} 0.20 & {\cellcolor[HTML]{D4DDE9}} 0.57 & {\cellcolor[HTML]{DFE5ED}} 0.38 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{F1E6E9}} 1.65 & {\cellcolor[HTML]{F2EFEF}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
mt\_minde\_imp\_s & {\cellcolor[HTML]{F2F2F2}} 0.21 & {\cellcolor[HTML]{F2ECED}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.27 & {\cellcolor[HTML]{F2F2F2}} 0.47 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{4479BB}} 2.25 & {\cellcolor[HTML]{EFF0F2}} 1.05 & {\cellcolor[HTML]{DCE3EC}} 1.11 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{4479BB}} 2.14 & {\cellcolor[HTML]{4479BB}} 2.22 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{ECEEF1}} 1.06 & {\cellcolor[HTML]{EFF0F2}} 0.62 & {\cellcolor[HTML]{4479BB}} 4.40 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{4479BB}} 2.09 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{E9ECF0}} 1.07 & {\cellcolor[HTML]{4479BB}} 1.95 & {\cellcolor[HTML]{E8B4C3}} 0.80 & {\cellcolor[HTML]{EABDCA}} 0.83 & {\cellcolor[HTML]{4479BB}} 2.14 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{ECEEF1}} 1.06 & {\cellcolor[HTML]{F2F2F2}} 0.20 & {\cellcolor[HTML]{EFDFE3}} 0.35 & {\cellcolor[HTML]{EFF0F2}} 0.22 & {\cellcolor[HTML]{DFE5ED}} 0.37 & {\cellcolor[HTML]{F2F2F2}} 0.20 & {\cellcolor[HTML]{D4DDE9}} 0.57 & {\cellcolor[HTML]{E4E8EE}} 0.37 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F1E9EB}} 1.66 & {\cellcolor[HTML]{F2EFEF}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
%c\_minde & {\cellcolor[HTML]{F2EFEF}} 0.19 & {\cellcolor[HTML]{EFDFE3}} 0.35 & {\cellcolor[HTML]{F1E6E9}} 0.23 & {\cellcolor[HTML]{F1E6E9}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{D7DFEA}} 1.13 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{BFCEE2}} 1.21 & {\cellcolor[HTML]{DCE3EC}} 1.38 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 0.58 & {\cellcolor[HTML]{F2F2F2}} 1.63 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{D1DBE8}} 1.15 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{E7AABB}} 0.77 & {\cellcolor[HTML]{E59EB2}} 0.73 & {\cellcolor[HTML]{D4DDE9}} 1.14 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{F0E3E7}} 0.15 & {\cellcolor[HTML]{F2F2F2}} 0.45 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{F2EFEF}} 0.15 & {\cellcolor[HTML]{F2ECED}} 0.41 & {\cellcolor[HTML]{F1E9EB}} 0.25 & {\cellcolor[HTML]{E8AFC0}} 0.18 & {\cellcolor[HTML]{F0E3E7}} 1.64 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
c\_minde\_imp & {\cellcolor[HTML]{F2EFEF}} 0.19 & {\cellcolor[HTML]{EFDFE3}} 0.35 & {\cellcolor[HTML]{F1E6E9}} 0.23 & {\cellcolor[HTML]{F1E6E9}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{D7DFEA}} 1.13 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{C1D0E3}} 1.20 & {\cellcolor[HTML]{DAE1EB}} 1.39 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 0.57 & {\cellcolor[HTML]{F2F2F2}} 1.60 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{D4DDE9}} 1.14 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{E6A3B7}} 0.75 & {\cellcolor[HTML]{E49AAF}} 0.72 & {\cellcolor[HTML]{D7DFEA}} 1.13 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{F1E6E9}} 0.16 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F2EFEF}} 0.26 & {\cellcolor[HTML]{F2F2F2}} 0.16 & {\cellcolor[HTML]{F2EFEF}} 0.42 & {\cellcolor[HTML]{F2ECED}} 0.26 & {\cellcolor[HTML]{EABDCA}} 0.22 & {\cellcolor[HTML]{EFDFE3}} 1.63 & {\cellcolor[HTML]{F2EFEF}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.40 \\
%c\_minde\_s & {\cellcolor[HTML]{F2F2F2}} 0.20 & {\cellcolor[HTML]{F0E3E7}} 0.36 & {\cellcolor[HTML]{F1E9EB}} 0.24 & {\cellcolor[HTML]{F1E9EB}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{C1D0E3}} 1.20 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{BFCEE2}} 1.21 & {\cellcolor[HTML]{F2F2F2}} 1.27 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2ECED}} 0.55 & {\cellcolor[HTML]{E4E8EE}} 1.69 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{BCCCE1}} 1.22 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{E6A3B7}} 0.75 & {\cellcolor[HTML]{E497AD}} 0.71 & {\cellcolor[HTML]{BFCEE2}} 1.21 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{F2ECED}} 0.18 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F2F2F2}} 0.18 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F2F2F2}} 0.47 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{F1E9EB}} 0.36 & {\cellcolor[HTML]{ECCAD4}} 1.56 & {\cellcolor[HTML]{F1E9EB}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
c\_minde\_imp\_s & {\cellcolor[HTML]{F2EFEF}} 0.19 & {\cellcolor[HTML]{F1E6E9}} 0.37 & {\cellcolor[HTML]{F1E9EB}} 0.24 & {\cellcolor[HTML]{F2ECED}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{C4D2E4}} 1.19 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{C1D0E3}} 1.20 & {\cellcolor[HTML]{F2F2F2}} 1.27 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2EFEF}} 0.56 & {\cellcolor[HTML]{DFE5ED}} 1.70 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{BFCEE2}} 1.21 & {\cellcolor[HTML]{EFDFE3}} 0.94 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{F2F2F2}} 1.04 & {\cellcolor[HTML]{E6A3B7}} 0.75 & {\cellcolor[HTML]{E59EB2}} 0.73 & {\cellcolor[HTML]{C1D0E3}} 1.20 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{EFDCE1}} 0.93 & {\cellcolor[HTML]{F2ECED}} 0.18 & {\cellcolor[HTML]{F0E3E7}} 0.36 & {\cellcolor[HTML]{F2F2F2}} 0.18 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{F2F2F2}} 0.17 & {\cellcolor[HTML]{F2F2F2}} 0.46 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{F1E6E9}} 0.35 & {\cellcolor[HTML]{EED6DD}} 1.60 & {\cellcolor[HTML]{F2EFEF}} 0.30 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
\midrule
MINE & {\cellcolor[HTML]{F2F2F2}} 0.23 & {\cellcolor[HTML]{F1E9EB}} 0.38 & {\cellcolor[HTML]{EED9DF}} 0.19 & {\cellcolor[HTML]{E6A7B9}} 0.19 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{E9BAC8}} 0.82 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{F2EFEF}} 1.26 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.58 & {\cellcolor[HTML]{F2EFEF}} 1.59 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E8AFC0}} 0.79 & {\cellcolor[HTML]{EED6DD}} 0.91 & {\cellcolor[HTML]{ECCAD4}} 0.87 & {\cellcolor[HTML]{E497AD}} 0.71 & {\cellcolor[HTML]{DF7D9A}} 0.63 & {\cellcolor[HTML]{DE7493}} 0.60 & {\cellcolor[HTML]{E7ADBE}} 0.78 & {\cellcolor[HTML]{ECCAD4}} 0.87 & {\cellcolor[HTML]{EBC2CE}} 0.85 & {\cellcolor[HTML]{EBC2CE}} 0.05 & {\cellcolor[HTML]{DF7B98}} 0.03 & {\cellcolor[HTML]{F1E9EB}} 0.14 & {\cellcolor[HTML]{ECCDD6}} 0.15 & {\cellcolor[HTML]{F0E3E7}} 0.11 & {\cellcolor[HTML]{E290A8}} 0.12 & {\cellcolor[HTML]{E8B4C3}} 0.08 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 1.69 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.42 \\
InfoNCE & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2ECED}} 0.39 & {\cellcolor[HTML]{EFDCE1}} 0.20 & {\cellcolor[HTML]{E8B4C3}} 0.23 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{E28BA4}} 0.67 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{E6A3B7}} 0.75 & {\cellcolor[HTML]{EFDFE3}} 1.21 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.58 & {\cellcolor[HTML]{E9B7C6}} 1.41 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E0809C}} 0.64 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{DC6A8C}} 0.57 & {\cellcolor[HTML]{E28EA6}} 0.68 & {\cellcolor[HTML]{DE7795}} 0.61 & {\cellcolor[HTML]{DF7B98}} 0.62 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{EBC6D1}} 0.86 & {\cellcolor[HTML]{F1E6E9}} 0.16 & {\cellcolor[HTML]{E7AABB}} 0.18 & {\cellcolor[HTML]{F2ECED}} 0.15 & {\cellcolor[HTML]{F0E3E7}} 0.22 & {\cellcolor[HTML]{F1E6E9}} 0.12 & {\cellcolor[HTML]{EBC2CE}} 0.28 & {\cellcolor[HTML]{EBC6D1}} 0.14 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 1.69 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
D-V & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2ECED}} 0.39 & {\cellcolor[HTML]{EED9DF}} 0.19 & {\cellcolor[HTML]{E8AFC0}} 0.22 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E5A1B5}} 0.74 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{E9B7C6}} 0.81 & {\cellcolor[HTML]{F1E9EB}} 1.24 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.58 & {\cellcolor[HTML]{EFDFE3}} 1.54 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E393AB}} 0.70 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{DF7D9A}} 0.63 & {\cellcolor[HTML]{E28BA4}} 0.67 & {\cellcolor[HTML]{DE7493}} 0.60 & {\cellcolor[HTML]{E290A8}} 0.69 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{EBC6D1}} 0.86 & {\cellcolor[HTML]{DB6487}} -0.25 & {\cellcolor[HTML]{D53D69}} -4.79 & {\cellcolor[HTML]{ECCDD6}} 0.05 & {\cellcolor[HTML]{E7AABB}} 0.04 & {\cellcolor[HTML]{EED9DF}} 0.08 & {\cellcolor[HTML]{D53D69}} -0.65 & {\cellcolor[HTML]{E8AFC0}} 0.07 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2F2F2}} 1.69 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
NWJ & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{F2ECED}} 0.39 & {\cellcolor[HTML]{EED9DF}} 0.19 & {\cellcolor[HTML]{E7ADBE}} 0.21 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E49AAF}} 0.72 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F1E9EB}} 0.97 & {\cellcolor[HTML]{F2F2F2}} 1.00 & {\cellcolor[HTML]{F2F2F2}} 0.28 & {\cellcolor[HTML]{E8B4C3}} 0.80 & {\cellcolor[HTML]{F1E9EB}} 1.24 & {\cellcolor[HTML]{F2EFEF}} 0.99 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2ECED}} 0.98 & {\cellcolor[HTML]{F2F2F2}} 0.58 & {\cellcolor[HTML]{EED9DF}} 1.52 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E59EB2}} 0.73 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{ECCDD6}} 0.88 & {\cellcolor[HTML]{E188A2}} 0.66 & {\cellcolor[HTML]{E28BA4}} 0.67 & {\cellcolor[HTML]{DD7191}} 0.59 & {\cellcolor[HTML]{E49AAF}} 0.72 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{EBC6D1}} 0.86 & {\cellcolor[HTML]{DB6185}} -0.26 & {\cellcolor[HTML]{D53D69}} -0.21 & {\cellcolor[HTML]{D53D69}} -44.48 & {\cellcolor[HTML]{E9B7C6}} 0.08 & {\cellcolor[HTML]{EDD0D8}} 0.05 & {\cellcolor[HTML]{DE7493}} 0.03 & {\cellcolor[HTML]{E8AFC0}} 0.07 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{F2EFEF}} 1.68 & {\cellcolor[HTML]{F2F2F2}} 0.32 & {\cellcolor[HTML]{F2F2F2}} 0.41 \\
KSG & {\cellcolor[HTML]{F2F2F2}} 0.22 & {\cellcolor[HTML]{EFDFE3}} 0.35 & {\cellcolor[HTML]{EED3DB}} 0.17 & {\cellcolor[HTML]{E9B7C6}} 0.24 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{D53D69}} 0.14 & {\cellcolor[HTML]{EABDCA}} 0.83 & {\cellcolor[HTML]{DE7795}} 0.61 & {\cellcolor[HTML]{F2F2F2}} 1.03 & {\cellcolor[HTML]{F2F2F2}} 0.30 & {\cellcolor[HTML]{D53D69}} 0.16 & {\cellcolor[HTML]{E7AABB}} 1.04 & {\cellcolor[HTML]{EED9DF}} 0.92 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{E28EA6}} 0.68 & {\cellcolor[HTML]{F2ECED}} 0.55 & {\cellcolor[HTML]{E1849F}} 1.25 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{D53D69}} 0.17 & {\cellcolor[HTML]{EDD0D8}} 0.89 & {\cellcolor[HTML]{E28BA4}} 0.67 & {\cellcolor[HTML]{D53D69}} 0.15 & {\cellcolor[HTML]{E1849F}} 0.65 & {\cellcolor[HTML]{D9557C}} 0.50 & {\cellcolor[HTML]{D53D69}} 0.17 & {\cellcolor[HTML]{ECCAD4}} 0.87 & {\cellcolor[HTML]{E0809C}} 0.64 & {\cellcolor[HTML]{EFDFE3}} 0.14 & {\cellcolor[HTML]{E7ADBE}} 0.19 & {\cellcolor[HTML]{EED6DD}} 0.08 & {\cellcolor[HTML]{EAC0CC}} 0.11 & {\cellcolor[HTML]{EED6DD}} 0.07 & {\cellcolor[HTML]{E7ADBE}} 0.21 & {\cellcolor[HTML]{ECCDD6}} 0.16 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2ECED}} 1.67 & {\cellcolor[HTML]{F2F2F2}} 0.31 & {\cellcolor[HTML]{F2F2F2}} 0.42 \\
LNN & {\cellcolor[HTML]{EFF0F2}} 0.25 & {\cellcolor[HTML]{5585C0}} 0.97 & {\cellcolor[HTML]{4479BB}} 2.85 & {\cellcolor[HTML]{4479BB}} 6.48 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{F2F2F2}} 0.43 & {\cellcolor[HTML]{4479BB}} 17.20 & {\cellcolor[HTML]{4479BB}} 2.77 & {\cellcolor[HTML]{4479BB}} 6.29 & {\cellcolor[HTML]{9AB4D6}} 1.33 & {\cellcolor[HTML]{749ACA}} 0.73 & {\cellcolor[HTML]{4479BB}} 17.20 & {\cellcolor[HTML]{4479BB}} 17.20 & {\cellcolor[HTML]{4479BB}} 3.25 & {\cellcolor[HTML]{4479BB}} 2.65 & {\cellcolor[HTML]{4479BB}} 7.04 & {\cellcolor[HTML]{4479BB}} 6.59 & {\cellcolor[HTML]{4479BB}} 33.40 & {\cellcolor[HTML]{F2F2F2}} 0.40 & {\cellcolor[HTML]{4479BB}} 17.20 & {\cellcolor[HTML]{4479BB}} 2.71 & {\cellcolor[HTML]{4479BB}} 7.03 & {\cellcolor[HTML]{4479BB}} 17.20 & {\cellcolor[HTML]{4479BB}} 3.26 & {\cellcolor[HTML]{4479BB}} 7.04 & {\cellcolor[HTML]{4479BB}} 17.20 & {\cellcolor[HTML]{4479BB}} 2.60 & {\cellcolor[HTML]{4479BB}} 7.00 & {\cellcolor[HTML]{DE7493}} -0.20 & {\cellcolor[HTML]{D53D69}} -0.56 & {\cellcolor[HTML]{7FA2CE}} 0.59 & {\cellcolor[HTML]{4479BB}} 1.39 & {\cellcolor[HTML]{4479BB}} 2.24 & {\cellcolor[HTML]{4479BB}} 3.03 & {\cellcolor[HTML]{4479BB}} 5.47 & {\cellcolor[HTML]{F1E9EB}} 0.36 & {\cellcolor[HTML]{E6A7B9}} 1.45 & {\cellcolor[HTML]{F2ECED}} 0.29 & {\cellcolor[HTML]{F2F2F2}} 0.43 \\
CCA & {\cellcolor[HTML]{E8B4C3}} 0.00 & {\cellcolor[HTML]{DD7191}} 0.00 & {\cellcolor[HTML]{E59EB2}} 0.00 & {\cellcolor[HTML]{DD6F8F}} 0.01 & {\cellcolor[HTML]{F0E3E7}} 0.34 & {\cellcolor[HTML]{F2F2F2}} 0.42 & {\cellcolor[HTML]{F2EFEF}} 0.38 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F0E3E7}} 0.95 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.29 & {\cellcolor[HTML]{E6EAEF}} 1.08 & {\cellcolor[HTML]{E4E8EE}} 1.36 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F2F2F2}} 0.41 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{F2F2F2}} 0.60 & {\cellcolor[HTML]{AAC0DC}} 1.88 & {\cellcolor[HTML]{F2F2F2}} 0.39 & {\cellcolor[HTML]{F2F2F2}} 1.02 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{F1E6E9}} 0.96 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{D53D69}} 0.24 & {\cellcolor[HTML]{D53D69}} 0.38 & {\cellcolor[HTML]{F2F2F2}} 1.01 & {\cellcolor[HTML]{EAC0CC}} 0.84 & {\cellcolor[HTML]{EED3DB}} 0.90 & {\cellcolor[HTML]{97B3D5}} 0.54 & {\cellcolor[HTML]{4479BB}} 2.21 & {\cellcolor[HTML]{EDD0D8}} 0.06 & {\cellcolor[HTML]{EAC0CC}} 0.11 & {\cellcolor[HTML]{EBC2CE}} 0.01 & {\cellcolor[HTML]{EED9DF}} 0.35 & {\cellcolor[HTML]{E5A1B5}} 0.02 & {\cellcolor[HTML]{DF7D9A}} 0.02 & {\cellcolor[HTML]{EFDFE3}} 1.63 & {\cellcolor[HTML]{ECCAD4}} 0.18 & {\cellcolor[HTML]{F2EFEF}} 0.38 \\dist & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\
\bottomrule
\end{tabular}

\caption{Mean estimate over 5 seeds using N = 5000 samples compared each against the ground-truth. Our method and all neural estimators were trained with 5000 training samples. List of abbreviations ( \textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral)
}

\end{table}

